Leveraging Pre-trained Large Language Models to Construct and Utilize World Models for Model-based Task Planning

There is a growing interest in applying pre-trained large language models (LLMs) to planning problems. However, methods that use LLMs directly as planners are currently impractical due to several factors, including limited correctness of plans, strong reliance on feedback from interactions with simulators or even the actual environment, and the inefficiency in utilizing human feedback. In this work, we introduce a novel alternative paradigm that constructs an explicit world (domain) model in planning domain definition language (PDDL) and then uses it to plan with sound domain-independent planners. To address the fact that LLMs may not generate a fully functional PDDL model initially, we employ LLMs as an interface between PDDL and sources of corrective feedback, such as PDDL validators and humans. For users who lack a background in PDDL, we show that LLMs can translate PDDL into natural language and effectively encode corrective feedback back to the underlying domain model. Our framework not only enjoys the correctness guarantee offered by the external planners but also reduces human involvement by allowing users to correct domain models at the beginning, rather than inspecting and correcting (through interactive prompting) every generated plan as in previous work. On two IPC domains and a Household domain that is more complicated than commonly used benchmarks such as ALFWorld, we demonstrate that GPT-4 can be leveraged to produce high-quality PDDL models for over 40 actions, and the corrected PDDL models are then used to successfully solve 48 challenging planning tasks. Resources, including the source code, are released at: https://guansuns.github.io/pages/llm-dm.

==> results/examples/pddl_example.tex <==
(:action PutDownBlock
   :parameters (?x - block)
   :precondition (and (robot-holding ?x))
   :effect (and (not (robot-holding ?x)) (block-clear ?x) (robot-hand-empty) (block-on-table ?x)))

==> results/household_action_description/close.tex <==
This action enables the robot to close a large piece of furniture (e.g., cabinets and drawers) or an appliance (e.g., dishwashers and refrigerators) that is openable. For example, the robot closes cabinet_1, or the robot closes drawer_2.

==> results/household_action_description/close_small.tex <==
This action enables the robot to close a small receptacle receptacle_1 that is openable (e.g. small storage boxes or lunch boxes with lids). For example, the robot closes lunch_box_2, or the robot closes storage_box_1.

==> results/household_action_description/empty_vacuum.tex <==
This action enables the robot to empty a vacuum cleaner’s dust bin and dump the dust into a trash can. For example, the robot empties vacuum_cleaner_1 and dumps the dust into trash_can_2, or the robot empties vacuum_cleaner_2 and dumps the dust into trash_can 1.

==> results/household_action_description/goto.tex <==
This action enables the robot to navigate from one normally immovable piece of furniture to another (e.g., dining tables, side tables, cabinets, and sinks) or an appliance (e.g., refrigerators, coffee makers, microwaves, and washers).

==> results/household_action_description/heat_microwave.tex <==
This action enables the robot to start a microwave and heat up the food inside. For example, the robot heats pizza_1 with microwave_2, the robot heats pasta_2 with microwave_1.

==> results/household_action_description/heat_pan.tex <==
This action enables the robot to heat food which is heatable with a pan. For example, the robot heats pizza_1 with pan_2, the robot heats pasta_2 with pan_1.

==> results/household_action_description/make_smoothie.tex <==
This action enables the robot to use a blender to make a smoothie by mashing and mixing all the food in the blender. For example, the robot gets apple_banana_smoothie_1 with blender_1, or the robot gets orange_banana_smoothie_1 with blender_2.

==> results/household_action_description/mash.tex <==
This action enables the robot to use a blender to mash some food in it. For example, the robot gets mashed apple_2 with blender_1, or the robot gets mashed banana_1 with blender_2.

==> results/household_action_description/open.tex <==
This action enables the robot to open a large piece of furniture (e.g., cabinets and drawers) or an appliance (e.g., dishwashers and refrigerators) that is openable. For example, the robot opens cabinet_1, or the robot opens drawer_2.

==> results/household_action_description/open_small.tex <==
This action enables the robot to open a small receptacle receptacle_1 (e.g. small storage boxes or lunch boxes with lids). For example, the robot opens lunch_box_2, or the robot opens storage_box_1.

==> results/household_action_description/pickup.tex <==
This action enables the robot to pick up an object object_1 in/on a large piece of furniture (e.g., dining tables, drawers, cabinets) or an appliance (e.g., dishwashers and refrigerators). For example, the robot pick up coffee_mug_1 on dining_table_1, the robot pick up fork_1 in drawer_1, or the robot pick up apple_1 in refrigerator_1.

==> results/household_action_description/pickup_small.tex <==
This action enables the robot to pick up an object object_1 in some small receptacle receptacle_1 (e.g. storage boxes, lunch boxes, bowls, plates). For example, the robot picks up apple_1 in blow_1, or the robot picks up apple_2 in lunch_box_2.

==> results/household_action_description/put.tex <==
This action enables the robot to put an object object_1 in/on a large piece of furniture (e.g., dining tables, drawers, cabinets) or an appliance (e.g., dishwashers and refrigerators). For example, the robot puts coffee_mug_1 on dining_table_1, the robot puts fork_1 in drawer_1, or the robot puts apple_1 in refrigerator_1.

==> results/household_action_description/put_small.tex <==
This action enables the robot to put an object object_1 into/onto a small receptacle receptacle_1 (e.g. storage boxes, bowls, plates, or pans). For example, the robot puts apple_1 into blow_1, or the robot puts apple_2 into lunch_box_2.

==> results/household_action_description/slice.tex <==
This action enables the robot to slice objects (like fruits and vegetables) with a knife. For example, the robot slices orange_1 with knife_2, the robot slices potato_3 with knife_1.

==> results/household_action_description/stack.tex <==
This action enables the robot to stack one object object_1 on top of another object object_2 that is on the same piece of furniture. For example, the robot stacks book_1 on top of book_2, or the robot stacks lunch_box_1 on top of lunch_box_2.

==> results/household_action_description/toggle_off.tex <==
This action enables the robot to toggle a small appliances (like humidifiers and light bulbs) to switch them off. For example, the robot toggles humidifier_2 off, or the robot toggle light_bulb_1 off.

==> results/household_action_description/toggle_on.tex <==
This action enables the robot to toggle a small appliances (like humidifiers and light bulbs) to switch them on. For example, the robot toggles humidifier_2 on, or the robot toggle light_bulb_1 on.

==> results/household_action_description/transfer.tex <==
This action enables the robot to transfer food food_1 from one small receptacle receptacle_1 to another small receptacle receptacle_2. This skill is usually used to transfer food that can not be easily picked up by the robot. For example, the robot can pour the milk from milk_box_1 to mug_1, or the robot can transfer heated pizza_1 from pan_2 to plate_1.

==> results/household_action_description/unstack.tex <==
This action enables the robot to unstack one object object_1 that is on top of another object object_2. For example, the robot stacks book_1 on top of book_2, or the robot stacks lunch_box_1 on top of lunch_box_2. The robot will hold the object after unstacking it.

==> results/household_action_description/vacuum.tex <==
This action enables the robot to vacuum a carpet with a handheld vacuum cleaner. For example, the robot uses vacuum_cleaner_1 to vacuum carpet_2, the robot uses vacuum_cleaner_2 to vacuum carpet_1.

==> results/household_action_description/wash.tex <==
This action enables the robot to wash an object (e.g., fruits and cloths) in a sink or basin. For example, the robot washed apple_1, or the robot washed romaine_lettuce_1.

==> results/household_action_description/wipe.tex <==
This action enables the robot to wipe and clean the surface of a piece of furniture or an appliance, such as a dining table, a mirror, a sink, or a bathtub, with a cloth. For example, the robot wipes dining_table_1 with cloth_1, the robot wipes mirror_1 with cloth_2.

==> results/household_extra_info/close_small.tex <==
(a) This action is only applicable for receptacles that are openable.
(b) The receptacle needs to be placed on a furniture piece that has an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).
(c) The receptacle should not be stacked on top of other objects if it is stackable.

==> results/household_extra_info/empty_vacuum.tex <==
(a) Note that the robot should hold the vacuum cleaner and stand by the trash can before executing this action.
(b) After executing this action, the robot is still holding the vacuum cleaner.
(c) The trash can should be opened if it's openable.
(d) The dust bin will be empty after executing this action.

==> results/household_extra_info/heat_microwave.tex <==
(a) The food to heat should be placed in a small receptacle (e.g., a plate or a bowl).
(b) The robot also needs to close the door of the microwave before taking this action.
(c) Note that the food is no longer pickupable after it has been heated.

==> results/household_extra_info/heat_pan.tex <==
(a) Note that the food should be placed on the pan, and the pan needs to be placed on a stove burner before executing this action. 
(b) A stove burner can be viewed as an immovable appliance, and a pan can be viewed as a small receptacle.
(c) Note that the food is no longer pickupable after it has been heated.

==> results/household_extra_info/mash.tex <==
(a) The food needs to be sliced beforehand and the food should be placed inside the blender.
(b) Note that the food remains in the blender after this action is performed.
(c) You may also assume the blender is turned off before and after mashing the food.

==> results/household_extra_info/open_small.tex <==
(a) This action is only applicable for receptacles that are openable.
(b) The receptacle needs to be placed on a furniture piece that has an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).
(c) The receptacle should not be stacked on top of other objects if it is stackable.

==> results/household_extra_info/pickup.tex <==
(a) This action is only applicable for objects that are pickupable by the robot.
(b) The furniture piece or appliance should be opened if it is openable.
(c) The object to pick up should not be stacked on top of other household items.

==> results/household_extra_info/pickup_small.tex <==
(a) The furniture piece needs to have an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).
(b) The receptacle should be opened if it is openable.

==> results/household_extra_info/put.tex <==
(a) The furniture piece or appliance should be opened if it is openable.

==> results/household_extra_info/put_small.tex <==
(a) The furniture piece needs to have an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).
(b) The receptacle should be opened if it is openable.
(c) The receptacle should not be stacked on top of other objects if it is stackable.

==> results/household_extra_info/slice.tex <==
(a) Note that the object to slice needs to be placed on a cutting board. A cutting board can be viewed as a special kind of receptacle.
(b) You may assume the robot is holding the knife in its gripper at the beginning.
(c) The object to slice should be sliceable.
(d) The furniture piece needs to have an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).

==> results/household_extra_info/stack.tex <==
(a) The furniture piece has to have an open and flat surface.
(b) Note that both object_1 and object_2 must be stackable objects.
(c) You may assume the robot is holding object_1 at the beginning.
(d) Also, there should be no other object on top of object_2.

==> results/household_extra_info/transfer.tex <==
(a) The furniture piece needs to have an open and flat surface to allow enough space for manipulation (e.g., countertops or tables).
(b) A receptacle should be opened if it is openable.
(c) Both receptacles should not be stacked on top of other objects if they are stackable.

==> results/household_extra_info/vacuum_carpet.tex <==
(a) You need to make sure the dust bin of the vacuum cleaner is not full before executing this action.
(b) You may assume the robot is holding the vacuum cleaner at the beginning.
(c) The dust bin of the vacuum cleaner will be full of dust.

==> results/household_extra_info/wash.tex <==
(a) The object has to be something washable.
(b) The robot should hold the object when washing it.

==> results/household_extra_info/wipe.tex <==
(a) You may assume the robot is holding the cloth before executing this action.
(b) The cloth will be dirty after executing the action.
(c) The robot should also use a clean cloth.

==> results/household_gpt35_correction/slice.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?x - householdObject: the object to slice
2. ?k - householdObject: the knife to use for slicing
3. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
|\highlight{\warningcolor}{Incorrect object type, a cutting board should be viewed as}|
|\highlight{\warningcolor}{    a small receptacle as mentioned in the prompt}|
4. ?z - householdObject: the cutting board on which the object is placed

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be on the cutting board not directly on the furniture ?y}|
    (object-on ?x ?y)
    (object-on ?z ?y)
    (robot-holding ?k)
    (sliceable ?x)
    (cutting-board ?z)
    (knife ?k)
    (flat-surface ?y)
    (object-whole ?x)
)

Effects:
(and
    (not (object-whole ?x))
    (object-sliced ?x)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There are some errors in the PDDL model:
1. There is an incorrect object type: a cutting board should be viewed as a small receptacle as mentioned in the prompt
2. There is an incorrect precondition: ?x should be on the cutting board not directly on the furniture ?y

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-3.5-Turbo:}|
1. ?x - householdObject: the object to slice
2. ?k - householdObject: the knife to use for slicing
3. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
4. ?z - smallReceptacle: the cutting board on which the object is placed

Preconditions:
(and
    (robot-at ?y)
    (object-on ?z ?y)
    (object-in ?x ?z)
    (robot-holding ?k)
    (sliceable ?x)
    |\highlight{\warningcolor}{Should use the predicate (cutting-board ?z)}|
    (is-small-receptacle ?z)
    (knife ?k)
    (flat-surface ?y)
    (object-whole ?x)
)

Effects:
(and
    (not (object-whole ?x))
    (object-sliced ?x)
)

==> results/household_gpt35_pddl/close.tex <==
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to close


Preconditions:
(and
    (robot-at ?x)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (connected ?x ?y)
    (robot-hand-empty)
    (open ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?obj not listed as parameter}|
    (not (on ?obj ?x))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (turned-on ?x))
    |\highlight{\warningcolor}{Incorrect precondition: ?obj not listed as parameter}|
    (not (robot-holding ?obj))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (turned-off ?x))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (cleaned ?x))
)

Effects:
(and
    (not (open ?x))
    |\highlight{\minorcolor}{Unnecessary effect: only changed predicates can be listed}|
    (robot-hand-empty)
    |\highlight{\warningcolor}{Incorrect effect: ?x need not be cleaned}|
    (cleaned ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to close

Preconditions:
(and
    (robot-at ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?y not listed as parameter}|
    (connected ?x ?y)
    |\highlight{\warningcolor}{Incorrect precondition: invalid predicate design}|
    (robot-holding nothing)
    (open ?x)
    |\highlight{\minorcolor}{Irrelevant precondition}|
    (not (smallAppliance ?x))
    
)

Effects:
(and
    (not (open ?x))
)

==> results/household_gpt35_pddl/close_small.tex <==
Parameters:
1. ?x - householdObject: the small receptacle to close
|\highlight{\warningcolor}{Missing parameter: ?z where the small receptacle is placed}|

Preconditions:
(and
    |\highlight{\warningcolor}{Unknown parameter ?y}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Unknown parameter ?y}|
    (connected ?y ?z)
    (on ?x ?z)
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (open ?z)
    |\highlight{\warningcolor}{Incorrect precondition: robot should have hand empty}|
    (not (robot-holding ?obj))
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be a small receptacle}|
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be closed}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x needs to be closed}|
    (not (open ?z))
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the small receptacle to close
|\highlight{\warningcolor}{Missing parameter: ?z where the small receptacle is placed}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Incorrect precondition and invalid use of the predicate}|
    (connected ?y ?z - furnitureAppliance)
    (on ?x ?z)
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?z needs to be a flat surface}|
    (openable ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?z needs to be a flat surface}|
    (open ?z)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (pickupable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be a small receptacle}|
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be closed}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x needs to be closed}|
    (not (open ?z))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (on ?x ?z))
    |\highlight{\warningcolor}{Irrelevant effect}|
    (not (robot-holding ?x))
    |\highlight{\minorcolor}{Irrelevant effect}|
    (robot-hand-empty)
)

==> results/household_gpt35_pddl/empty_vacuum.tex <==
Parameters:
1. ?vacuum - householdObject: the vacuum cleaner to empty
2. ?trash - furnitureAppliance: the trash can to dump the dust into

Preconditions:
(and
    (robot-at ?trash)
    (robot-holding ?vacuum)
    |\highlight{\warningcolor}{Invalid predicate}|
    (smallAppliance ?vacuum)
    (turned-off ?vacuum)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (cleaned ?vacuum)
    |\highlight{\warningcolor}{Missing precondition: ?vacuum is a vacuum}|
    |\highlight{\warningcolor}{Missing precondition: ?trash is a trash can}|
)

Effects:
(and
    (not (robot-holding ?vacuum))
    (on ?vacuum ?trash)
    |\highlight{\warningcolor}{Missing effect: the dust bin of ?vacuum is empty}|
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the vacuum cleaner to empty
2. ?y - furnitureAppliance: the trash can to dump the dust into

Preconditions:
(and
    (robot-at ?y)
    (robot-holding ?x)
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (pickupable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x is held by robot}|
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (openable ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (open ?y)
    |\highlight{\warningcolor}{Missing precondition: the dust bin of ?x is full}|
    |\highlight{\warningcolor}{Missing precondition: ?x is a vacuum}|
    |\highlight{\warningcolor}{Missing precondition: ?y is a trash can}|
)

Effects:
(and
    |\highlight{\warningcolor}{Inaccurate effect}|
    (not (dirty ?x))
    (robot-holding ?x)
    |\highlight{\warningcolor}{Missing effect: the dust bin of ?x is empty}|
)

==> results/household_gpt35_pddl/goto.tex <==
Parameters:
1. ?f1 - furnitureAppliance: the furniture/appliance to navigate from
2. ?f2 - furnitureAppliance: the furniture/appliance to navigate to

Preconditions:
(and
    (robot-at ?f1)
    (reachable ?f1 ?f2)
    |\highlight{\warningcolor}{Irrelevant preconditions}|
    (not (robot-holding ?o))
    |\highlight{\warningcolor}{Irrelevant preconditions}|
    (forall (?o - householdObject)
        (not (object-on ?o ?f1))
    )
)

Effects:
(and
    (robot-at ?f2)
    |\highlight{\warningcolor}{Missing effect: (not (robot-at ?f1))}|
)

==> results/household_gpt35_pddl/heat_microwave.tex <==
Parameters:
1. ?x - householdObject: the object to heat up
2. ?y - furnitureAppliance: the microwave to use

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?z not a parameter}|
    (connected ?y ?z)
    |\highlight{\warningcolor}{Incorrect precondition: robot can't be at two places at once}|
    (robot-at ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on ?x ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    (open ?y)
    (turned-on ?y)
    (not (robot-holding ?x))
    (not (turned-off ?y))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (cleaned ?y))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (smallAppliance ?x))
    |\highlight{\warningcolor}{Missing precondition: ?y is a microwave}|
    |\highlight{\warningcolor}{Missing precondition: robot should not hold anything}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?z is not a parameter}|
    (not (on ?x ?z))
    (robot-holding ?x)
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (on-table ?y))
    |\highlight{\warningcolor}{Missing effect: ?x is heated}|
    
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the food to heat up
2. ?y - furnitureAppliance: the microwave to use
|\highlight{\warningcolor}{Missing parameter: ?r - small receptacle where ?x is placed}|

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y and ?x can't be connected}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be in a small receptacle}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (not (robot-holding knife))
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (openable ?y)
    (not (open ?y))
    |\highlight{\warningcolor}{Invalid predicate design}|
    (robot-holding nothing)
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (pickupable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x-sliced not a parameter}|
    (not (pickupable ?x-sliced))
    (not (robot-holding ?x-sliced))
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be clean}|
    (not (dirty ?x))
    |\highlight{\minorcolor}{Unnecessary precondition: This is already implied}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Missing precondition: robot should not hold anything}|
    |\highlight{\warningcolor}{Missing precondition: ?y is a microwave}|
    |\highlight{\warningcolor}{Missing precondition: ?r is a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?r should be in ?y}|
)

Effects:
(and
    (not (open ?y))
    (not (pickupable ?x))
    (not (robot-holding ?x))
    (turned-on ?y)
    |\highlight{\warningcolor}{Incorrect effect: robot can have hand-empty}|
    (not (robot-hand-empty))
    |\highlight{\warningcolor}{Invalid predicate design}|
    (robot-holding nothing)
    |\highlight{\warningcolor}{Syntax error: ?x-sliced not a parameter}|
    (not (pickupable ?x-sliced))
    |\highlight{\warningcolor}{Syntax error: ?x-sliced not a parameter}|
    (not (robot-holding ?x-sliced))
    |\highlight{\warningcolor}{Missing effect: ?x is heated}|
)


==> results/household_gpt35_pddl/heat_pan.tex <==
Parameters:
1. ?x - householdObject: the object to heat
|\highlight{\warningcolor}{Incorrect parameter: ?y should be a householdObject}|
2. ?y - furnitureAppliance: the pan to use for heating
|\highlight{\warningcolor}{Missing parameter: the stove burner where pan can be heated}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y and ?x aren't connected}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y need not be opened}|
    (open ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y is a pan}|
    (turned-on ?y)
    |\highlight{\warningcolor}{Invalid predicate design}|
    (robot-holding ?empty - nothing)
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (not (robot-holding ?x))
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (not (smallAppliance ?x))
    |\highlight{\warningcolor}{Missing precondition: ?y is on stove}|
    |\highlight{\warningcolor}{Missing precondition: ?y is a pan}|
)

Effects:
(and
    (not (on ?y ?x))
    |\highlight{\warningcolor}{Incorrect effect: ?x will not be pickupable}|
    (robot-holding ?x)
    |\highlight{\warningcolor}{Incorrect effect: ?y is a pan}|
    (not (turned-on ?y))
    |\highlight{\warningcolor}{Incorrect effect: ?empty is not a parameter}|
    (not (robot-holding ?empty))
    |\highlight{\warningcolor}{Missing effect: ?x is heated}|
    |\highlight{\warningcolor}{Missing effect: ?x is not pickupable}|
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the food to be heated
2. ?y - householdObject: the pan to be used for heating
|\highlight{\warningcolor}{Missing parameter: the stove where pan can be heated}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (connected ?z - furnitureAppliance ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (connected ?z - furnitureAppliance ?a - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?y - householdObject ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?a - householdObject ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on-table ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-holding nothing)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (pickupable ?x - householdObject)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?b - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (connected ?b - furnitureAppliance ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?y - householdObject ?b - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on-table ?b - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (pickupable ?y - householdObject)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?x - householdObject ?c - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?y - householdObject ?c - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (dirty ?y - householdObject))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    |\highlight{\warningcolor}{Other missing preconditions such as ?y should be a plan}|
)

Effects:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (robot-holding ?x - householdObject))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (pickupable ?x - householdObject))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (pickupable ?y - householdObject))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?x - householdObject ?z - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?y - householdObject ?z - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?x - householdObject ?a - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?y - householdObject ?a - furnitureAppliance))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (dirty ?y - householdObject))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?x-sliced - householdObject ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?y-sliced - householdObject ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-holding ?x-sliced - householdObject)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (turned-on ?z - smallAppliance)
    |\highlight{\warningcolor}{Missing effect: ?x is heated}|
    |\highlight{\warningcolor}{Missing effect: ?x is not pickupable}|
)

==> results/household_gpt35_pddl/mash.tex <==
Parameters:
1. ?x - householdObject: the object to be mashed
|\highlight{\warningcolor}{Incorrect object type: it should be ?householdObject}|
2. ?y - smallAppliance: the blender to use
|\highlight{\warningcolor}{Missing parameter: the furniture piece where the blender and food are placed}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on-table ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (open ?y)
    (turned-on ?y)
    |\highlight{\warningcolor}{Incorrect precondition: contradicts (on ?x ?y)}|
    (robot-holding ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?irrelevantObject is not a parameter}|
    (not (robot-holding ?irrelevantObject))
    |\highlight{\warningcolor}{Missing precondition: ?y should be a blender}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be on the same furniture piece as the robot}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: robot does not hold anything}|
    (not (robot-holding ?x))
    |\highlight{\warningcolor}{Incorrect effect: robot does not hold anything}|
    (robot-holding ?y)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (put-on ?x ?y)
    (not (cleaned ?y))
    |\highlight{\warningcolor}{Incorrect effect}|
    (smallAppliance ?y)
    |\highlight{\warningcolor}{Missing effect: ?x is mashed}|
    |\highlight{\warningcolor}{Missing effect: ?x is no longer pickupable}|
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the object to be mashed
|\highlight{\warningcolor}{Incorrect parameter: it is ?householdObject}|
2. ?y - furnitureAppliance: the blender to use
|\highlight{\warningcolor}{Missing parameter: the furniture piece where the blender and food are placed}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (on-table ?y)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (openable ?y)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (open ?y)
    (turned-off ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (robot-holding knife)
    (sliceable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x-sliced is not a parameter}|
    (on ?x-sliced ?y)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be clean}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x is sliced }|
    |\highlight{\warningcolor}{Missing precondition: ?y is a blender}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be on the same furniture piece as the robot}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x stays in ?y after action}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (on ?x-sliced ?y))
    |\highlight{\warningcolor}{Incorrect effect}|
    (robot-holding ?x-sliced)
    |\highlight{\warningcolor}{Missing effect: ?x is mashed}|
    |\highlight{\warningcolor}{Missing effect: ?x is no longer pickupable}|
)

==> results/household_gpt35_pddl/open.tex <==
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to open


Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect precondition: robot should be at ?x}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?z not listed as a parameter}|
    (not (robot-holding ?z))
    (not (open ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x should be openable}|
    |\highlight{\warningcolor}{Missing precondition: the robot shouldn't hold anything}|
)

Effects:
(and
    (open ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to open

Preconditions:
(and
    (robot-at ?x)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (connected ?x ?y)
    |\highlight{\warningcolor}{Invalid predicate design}|
    (robot-holding nothing)
    (openable ?x)
    (not (open ?x))
)

Effects:
(and
    (open ?x)
)


==> results/household_gpt35_pddl/open_small.tex <==
Parameters:
1. ?x - householdObject: the small receptacle to open
|\highlight{\warningcolor}{Missing parameter: ?y where the small receptacle is placed}|

Preconditions:
(and
    (robot-at ?y)
    (on ?x ?y)
    (on-table ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?z is not in parameter}|
    (not (robot-holding ?z))
    (not (open ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x needs to be openable}|
    |\highlight{\warningcolor}{Missing precondition: ?x should be a small receptacle}|
)

Effects:
(and
    (open ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the small receptacle to open
|\highlight{\warningcolor}{Missing parameter: ?z where the small receptacle is placed}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?z - furnitureAppliance)
    (on ?x ?z)
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?x needs to be openable not ?z}|
    (openable ?z)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Incorrect precondition: ?x-sliced is not needed}|
    (not (on ?x-sliced ?y))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (robot-holding ?x-sliced))
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (not (robot-holding nothing))
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be clean}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x should be a small receptacle}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x needs to be opened}|
    (open ?z)
)

==> results/household_gpt35_pddl/pickup.tex <==
Parameters:
1. ?o - householdObject: the object to pick up
2. ?f - furnitureAppliance: the furniture/appliance on which the object is located

Preconditions:
(and
    (robot-at ?f)
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameter: ?f1}|
    (reachable ?f1 ?f)
    (object-on ?o ?f)
    (object-pickupable ?o)
    |\highlight{\warningcolor}{Inaccurate precondition: "?x is not stacked on top of other object" should}|
    |\highlight{\warningcolor}{    only apply when ?x is a stackable object}|
    (not (object-stacked ?o))
    |\highlight{\warningcolor}{Inaccurate precondition: the gripper should be empty}|
    (not (robot-holding ?o))
    (or (not (furniture-openable ?f)) (furniture-open ?f))
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked}|
    |\highlight{\warningcolor}{    on top of ?x if ?x is a stackable object}|
)

Effects:
(and
    (not (object-on ?o ?f))
    |\highlight{\warningcolor}{Incorrect effect and unknown parameter: ?f1}|
    (not (object-in ?o ?c))
    |\highlight{\warningcolor}{Incorrect effect and unknown parameter: ?o2}|
    (not (object-stacked-on ?o ?o2))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-washed ?o))
    (robot-holding ?o)
)

==> results/household_gpt35_pddl/pickup_from_small.tex <==
Parameters:
1. ?x - householdObject: the object to pick up
|\highlight{\warningcolor}{Incorrect parameter: ?y should be a householdObject}|
2. ?y - furnitureAppliance: the small receptacle containing the object ?x
|\highlight{\warningcolor}{Missing parameter: ?z, the furniture piece where ?y is located}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect precondition: robot should be at furnitureAppliance}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?z)
    (robot-at ?z)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Incorrect parameter}|
    (on-table ?y)
    |\highlight{\warningcolor}{Inaccurate precondition: robot should hold nothing in its gripper}|
    (not (robot-holding ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x should be pickupable}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be opened if it is openable}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be on ?z}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Incorrect effect: robot won't move after the action}|
    (not (robot-at ?y))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (on-table ?y))
    (robot-holding ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the object to pick up
2. ?y - furnitureAppliance: the furniture or appliance containing the receptacle where the object is located
3. ?z - householdObject: the receptacle containing the object to pick up

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y and ?z need not be connected}|
    (connected ?y ?z)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?x ?z)
    (on-table ?y)
    |\highlight{\warningcolor}{Inaccurate precondition: ?z should be open if it is openable}|
    (openable ?z)
    |\highlight{\warningcolor}{Inaccurate precondition: ?z should be open if it is openable}|
    (open ?z)
    (pickupable ?x)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Incorrect precondition and incorrect use of the predicate}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (on ?x-sliced ?y))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (robot-holding ?x-sliced))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Missing precondition: ?z should be on ?y}|
    |\highlight{\warningcolor}{Missing precondition: ?z should be a small receptacle}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?z))
    |\highlight{\warningcolor}{Invalid predicate design}|
    (not (robot-holding nothing))
    (robot-holding ?x)
)
        

==> results/household_gpt35_pddl/predicates.tex <==
1. (robot-at ?f - furnitureAppliance): true if the robot is at furniture/appliance ?f
2. (reachable ?f1 - furnitureAppliance ?f2 - furnitureAppliance): true if furniture/appliance ?f2 is reachable from furniture/appliance ?f1. This predicate should be defined for each pair of reachable furniture/appliances.
3. (object-on ?o - householdObject ?f - furnitureAppliance): true if the object ?o is on/in the furniture/appliance ?f
4. (object-pickupable ?o - householdObject): true if the object ?o can be picked up by the robot
5. (object-stacked ?o - householdObject): true if the object ?o is stacked on top of another object
6. (furniture-openable ?f - furnitureAppliance): true if the furniture/appliance ?f can be opened
7. (furniture-open ?f - furnitureAppliance): true if the furniture/appliance ?f is open
8. (robot-holding ?o - householdObject): true if the robot is holding the object ?o
9. (object-stacked-on ?o1 - householdObject ?o2 - householdObject): true if the object ?o1 is stacked on top of the object ?o2
10. (smallAppliance ?a - householdObject): true if the object ?a is a small appliance
11. (furniture ?f - furnitureAppliance): true if the object ?f is a furniture/appliance
12. (smallContainer ?o - householdObject): true if the object ?o is a small container
13. (object-in ?o - householdObject ?f - furnitureAppliance): true if the object ?o is in/on the furniture/appliance ?f
14. (object-toggleable ?o - householdObject): true if the object ?o can be toggled on/off
15. (furniture-closed ?f - furnitureAppliance): true if the furniture/appliance ?f is closed.
16. (object-sliceable ?o - householdObject): true if the object ?o can be sliced
17. (object-sliced ?o - householdObject): true if the object ?o has been sliced
18. (object-on-cutting-board ?o - householdObject ?cb - furnitureAppliance): true if the object ?o is on the cutting board ?cb
19. (cutting-board-closed ?cb - furnitureAppliance): true if the cutting board ?cb is closed
20. (object-stacked-on ?o1 - householdObject ?o2 - householdObject): true if the object ?o1 is stacked on top of the object ?o2. This predicate is different from the one defined above as it is used to represent the effect of the action.
21. (smallContainer ?r - householdObject): true if the object ?r is a small container
22. (object-in ?o - householdObject ?r - householdObject): true if the object ?o is in/on the container ?r
23. (object-stacked-on ?o1 - householdObject ?o2 - householdObject): true if the object ?o1 is stacked on top of the object ?o2. This predicate is used to represent the precondition of the action.
24. (object-washed ?o - householdObject): true if the object ?o has been washed
25. (object-stacked-on ?o1 - householdObject ?o2 - householdObject): true if the object ?o1 is stacked on top of the object ?o2. This predicate is used to represent the effect of the action.
26. (object-in ?o - householdObject ?c - householdObject): true if the object ?o is in/on the container ?c

==> results/household_gpt35_pddl/prompt.tex <==
You are defining the preconditions and effects (represented in PDDL format) of a household robot's actions. Note that individual conditions in preconditions and effects should be listed separately.  For example, "object_1 is washed and heated" should be considered as two separate conditions "object_1 is washed" and "object_1 is heated". Also note that the robot has only one gripper, so (a) it can only hold one object, (b) it shouldn't hold any other irrelevant objects in its gripper while performing some manipulation tasks (e.g., opening a drawer or closing a window), (c) operations on small household items should be carried out on furniture with a flat surface to get enough space for manipulation. The robot can navigate to various large and normally immovable furniture pieces or appliances in the house to carry out household tasks.

There are two types of objects in this domain - one is the robot, the other is householdObject which captures all household items.

Here are two examples:

Example 1
Action: This action enables the robot to go to a normally immovable piece of furniture (e.g., dining tables, side tables, cabinets, and sinks) or an appliance (e.g., refrigerators, coffee makers, microwaves, and washers).

You can create and define new predicates, but you may also reuse the following predicates:
1. (object-at-furniture-appliance ?obj - householdObject ?furnitureAppliance - householdObject): true if the household item ?obj is in/on the furniture piece or appliance ?furnitureAppliance
2. (robot-at-furniture-appliance ?furnitureAppliance - householdObject): true if the robot is at the furniture piece or appliance ?furnitureAppliance
3. (robot-holding ?obj - householdObject): true if the robot is holding the household item ?obj
4. (is-furniture-appliance ?furnitureAppliance - householdObject): true if ?furnitureAppliance is a furniture piece or an appliance

Parameters:
1. ?furnitureAppliance1 - householdObject: current location of the robot
2. ?furnitureAppliance2 - householdObject: target location that the robot should go to

Preconditions:

(and
    (is-furniture-appliance ?furnitureAppliance1)
    (is-furniture-appliance ?furnitureAppliance2)
    (robot-at-furniture-appliance ?furnitureAppliance1)
    (not (robot-at-furniture-appliance ?furnitureAppliance2))
)


Effects:

(and
    (not (robot-at-furniture-appliance ?furnitureAppliance1))
    (robot-at-furniture-appliance ?furnitureAppliance2)
)


New Predicates:
No newly defined predicate


Example 2
Action: This action enables the robot to pick up an object object_1 in/on a large piece of furniture (e.g., dining tables, drawers, cabinets) or an appliance (e.g., dishwashers and refrigerators). For example, the robot puts coffee_mug_1 on dining_table_1, the robot puts fork_1 in drawer_1, or the robot puts apple_1 in refrigerator_1.

You can create and define new predicates, but you may also reuse the following predicates:
1. (object-at-furniture-appliance ?obj - householdObject ?furnitureAppliance - householdObject): true if the household item ?obj is in/on the furniture piece or appliance ?furnitureAppliance
2. (robot-at-furniture-appliance ?furnitureAppliance - householdObject): true if the robot is at the furniture piece or appliance ?furnitureAppliance
3. (robot-holding ?obj - householdObject): true if the robot is holding the household item ?obj
4. (robot-not-holding-anything): true if the robot is not holding anything in its gripper
5. (is-furniture-appliance ?furnitureAppliance - householdObject): true if ?furnitureAppliance is a furniture piece or an appliance

Parameters:
1. ?obj1 - householdObject: the object to pick up
2. ?furnitureAppliance1 - householdObject: the furniture or appliance where ?obj1 is located

Preconditions:

(and
    (is-furniture-appliance ?furnitureAppliance1)
    (robot-at-furniture-appliance ?furnitureAppliance1)
    (object-at-furniture-appliance ?obj1 ?furnitureAppliance1)
    (is-pickupable ?obj1)
    (robot-not-holding-anything)
    (or
        (not (openable-furniture-appliance ?furnitureAppliance1))
        (opened-furniture-appliance ?furnitureAppliance1)
    )
)


Effects:

(and
    (not (object-at-furniture-appliance ?obj1 ?furnitureAppliance1))
    (robot-holding ?obj1)
    (not (robot-not-holding-anything))
)


New Predicates:
1. (openable-furniture-appliance ?furnitureAppliance - householdObject): true if the furniture piece or appliance ?furnitureAppliance is openable (e.g., fridges, drawers, cabinets)
2. (opened-furniture-appliance ?furnitureAppliance - householdObject): true if the furniture piece or appliance ?furnitureAppliance is opened (e.g., fridges, drawers, cabinets)
3. (is-pickupable ?obj - householdObject): true if the household object ?obj is pickupable by the robot


Here is the task.


==> results/household_gpt35_pddl/put.tex <==
Parameters:
1. ?o - householdObject: the object to put in/on the furniture/appliance
2. ?f - furnitureAppliance: the furniture/appliance to put the object in/on

Preconditions:
(and
    (robot-at ?f)
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameter: ?f1}|
    (reachable ?f1 ?f)
    (object-pickupable ?o)
    |\highlight{\warningcolor}{Incorrect precondition: the robot should hold the object}|
    (not (robot-holding ?o))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (object-stacked ?o))
    (not (object-in ?o ?f))
    (not (object-on ?o ?f))
    (or (not (furniture-openable ?f)) (furniture-open ?f))
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameters}|
    (or (not (smallContainer ?o)) (object-in ?r ?f))
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameters}|
    (or (not (object-sliceable ?o)) (object-on-cutting-board ?o ?cb))
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameters}|
    (or (not (object-washed ?o)) (smallContainer ?r))
)

Effects:
(and
    (not (robot-holding ?o))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-on ?o ?f))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-in ?o ?f))
    (object-on ?o ?f)
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-stacked ?o))
    |\highlight{\warningcolor}{Incorrect effect}|
    (forall (?x - householdObject) (not (object-stacked-on ?x ?o)))
)

==> results/household_gpt35_pddl/put_into_small.tex <==
Parameters:
1. ?x - householdObject: the object to put into/onto the receptacle
|\highlight{\warningcolor}{Incorrect parameter: ?y should be householdObject}|
2. ?y - furnitureAppliance: the small receptacle to put the object into/onto
|\highlight{\warningcolor}{Missing parameter: ?z, the furniture piece where this action happens}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: connected is irrelevant to the action}|
    (connected ?y ?z)
    (robot-holding ?x)
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?irrelevant is not a parameter}|
    (not (robot-holding ?irrelevant))
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Incorrect precondition: ?y should be open if it is openable}|
    (not (open ?y))
    |\highlight{\minorcolor}{Irrelevant precondition}|
    (not (smallAppliance ?y))
    |\highlight{\warningcolor}{Missing precondition: ?y should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be on ?z}|
)

Effects:
(and
    (not (robot-holding ?x))
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (put-on ?x ?y)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the object to put into/onto the receptacle
2. ?y - furnitureAppliance: the furniture or appliance that has an open and flat surface to put the object onto
|\highlight{\warningcolor}{Incorrect parameter: ?z should be householdObject}|
3. ?z - furnitureAppliance: the small receptacle to put the object into/onto

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: connected is irrelevant to the action}|
    (connected ?y ?z)
    (on-table ?y)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (openable ?z)
    |\highlight{\warningcolor}{Inaccurate precondition: receptacle should be open if it is openable}|
    (open ?z)
    |\highlight{\warningcolor}{Incorrect precondition: robot should be holding ?x}|
    (not (robot-holding-something))
    (pickupable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: robot should be holding ?x}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?z))
    |\highlight{\warningcolor}{Missing precondition: ?z should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?z should be on ?y}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?x ?z)
    |\highlight{\warningcolor}{Invalid predicate design}|
    (robot-holding nothing)
)

==> results/household_gpt35_pddl/slice.tex <==
Parameters:
1. ?x - householdObject: the object to slice
2. ?y - householdObject: the knife to use for slicing
|\highlight{\warningcolor}{Missing parameter: ?furniture where the slicing takes place}|

Preconditions:
(and
    (robot-at ?furniture)
    (on ?x ?furniture)
    |\highlight{\warningcolor}{Incorrect precondition: ?y is held by the robot}|
    (on ?y ?furniture)
    (on-table ?furniture)
    (robot-holding ?y)
    |\highlight{\minorcolor}{Unnecessary precondition: (robot-holding ?y) implies this}|
    (not (robot-holding ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x should be sliceable}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be a knife}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x will be on ?furniture as the robot is holding the knife}|
    (not (on ?x ?furniture))
    |\highlight{\warningcolor}{Incorrect effect: ?x will be on ?furniture as the robot is holding the knife}|
    (robot-holding ?x)
    |\highlight{\warningcolor}{Missing effect: ?x should be sliced}|
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the object to slice
|\highlight{\warningcolor}{Incorrect object type, ?y should be householdObject}|
2. ?y - furnitureAppliance: the cutting board where the object is placed
|\highlight{\warningcolor}{Missing parameter ?knife}|
|\highlight{\warningcolor}{Missing parameter: the furniture where slicing takes place}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect precondition, the robot should be at a furniture piece}|
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-holding knife)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (robot-holding nothing)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on ?x ?y)
    |\highlight{\warningcolor}{Incorrect parameter, should be the furniture piece}|
    (on-table ?y)
    (sliceable ?x)
    |\highlight{\warningcolor}{Missing precondition: ?knife should be a knife}|
    |\highlight{\warningcolor}{Missing precondition: ?x should be on the cutting board}|
    |\highlight{\warningcolor}{Missing precondition: the cutting board should be on the furniture piece}|
    |\highlight{\warningcolor}{Missing precondition: ?y should be a cutting board}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?x ?y))
    |\highlight{\warningcolor}{Incorrect effect: ?x-sliced need not be created}|
    (on ?x-sliced ?y)
    (dirty ?y)
    |\highlight{\warningcolor}{Incorrect effect: ?x-sliced need not be created}|
    (robot-holding ?x-sliced)
    (not (robot-holding knife))
    (robot-holding-something)
    |\highlight{\warningcolor}{Missing effect: ?x should be sliced}|
    |\highlight{\warningcolor}{Missing effect: the location where ?knife is located}|
)

==> results/household_gpt35_pddl/stack.tex <==
1. ?object_1 - householdObject: the object to be stacked on top of another object
2. ?object_2 - householdObject: the object on which ?object_1 will be stacked
|\highlight{\warningcolor}{Missing parameter: ?f, the flat furniture piece}|

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error}|
    (robot-at ?f - furnitureAppliance)
    |\highlight{\warningcolor}{Syntax error and incorrect precondition}|
    (reachable ?f - furnitureAppliance ?f2 - furnitureAppliance)
    |\highlight{\warningcolor}{Incorrect precondition: should be stackable}|
    (object-pickupable ?object_1)
    |\highlight{\warningcolor}{Syntax error}|
    (object-stacked-on ?object_2 ?o - householdObject)
    |\highlight{\warningcolor}{Unnecessary precondition}|
    (not (object-stacked ?object_1))
    |\highlight{\warningcolor}{Unknown parameter}|
    (not (object-stacked-on ?o ?object_1))
    (object-on ?object_2 ?f)
    |\highlight{\warningcolor}{Incorrect precondition: the furniture piece should be flat not openable}|
    (furniture-openable ?f)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (furniture-open ?f)
    (robot-holding ?object_1)
    |\highlight{\warningcolor}{Missing precondition: there should be no other objects on top of ?object\_2}|
    |\highlight{\warningcolor}{Missing precondition: ?object\_2 should be stackable}|
)

Effects:
(and
    (not (robot-holding ?object_1))
    (object-stacked-on ?object_1 ?object_2)
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-on ?object_1 ?f))
)

==> results/household_gpt35_pddl/toggle_off.tex <==
Parameters:
|\highlight{\warningcolor}{Invalid object type: should be householdObject}|
1. ?x - smallAppliance: the small appliance to toggle off
|\highlight{\warningcolor}{Missing parameter: ?y - the furniture or appliance where ?x is located}|

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Irrelevant precondition and unknown parameters ?y \& ?z}|
    (connected ?y ?z)
    (on ?x ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?z need not be opened}|
    (open ?z)
    (turned-on ?x)
    |\highlight{\warningcolor}{Incorrect precondition: Invalid predicate design}|
    (robot-holding nothing)
)

Effects:
(and
    (not (turned-on ?x))
    (turned-off ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
|\highlight{\warningcolor}{Invalid object type: should be householdObject}|
1. ?x - smallAppliance: the small appliance to toggle off
|\highlight{\warningcolor}{Missing parameter: ?y - the furniture or appliance where ?x is located}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Irrelevant precondition and ?y not listed as parameter}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    (turned-on ?x)
    |\highlight{\warningcolor}{Invalid use of predicate}|
    (robot-holding nothing)
    |\highlight{\minorcolor}{Missing precondition: ?x should be at ?y}|
)

Effects:
(and
    (not (turned-on ?x))
    (turned-off ?x)
)

==> results/household_gpt35_pddl/toggle_on.tex <==
Parameters:
|\highlight{\warningcolor}{Invalid object type: should be householdObject}|
1. ?x - smallAppliance: the small appliance to toggle on
|\highlight{\warningcolor}{Missing parameter: ?y - the furniture or appliance where ?x is located}|

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?z not listed as parameter}|
    (not (robot-holding ?z))
    |\highlight{\warningcolor}{Incorrect predicate}|
    (not (open ?x))
    (not (turned-on ?x))
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be cleaned}|
    (cleaned ?x)
    |\highlight{\warningcolor}{Missing precondition: ?x should be at ?y}|
    |\highlight{\warningcolor}{Missing precondition: the robot should hold nothing in its gripper}|
)

Effects:
(and
    (turned-on ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
|\highlight{\warningcolor}{Invalid object type: should be householdObject}|
1. ?x - smallAppliance: the small appliance to toggle on
|\highlight{\warningcolor}{Missing parameter: ?y - the furniture or appliance the robot is currently at}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Incorrect precondition: ?y need not be openable}|
    (openable ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y need not be opened}|
    (open ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be pickupable}|
    (pickupable ?x)
    (on ?x ?y)
    (turned-off ?x)
    |\highlight{\warningcolor}{Missing precondition: the robot should hold nothing in its gripper}|
)

Effects:
(and
    (turned-on ?x)
    (not (turned-off ?x))
)

==> results/household_gpt35_pddl/transfer.tex <==
Parameters:
1. ?food - householdObject: the food to transfer
|\highlight{\warningcolor}{Incorrect parameter: receptacle should be a householdObject}|
2. ?receptacle1 - furnitureAppliance: the source receptacle
|\highlight{\warningcolor}{Incorrect parameter: receptacle should be a householdObject}|
3. ?receptacle2 - furnitureAppliance: the destination receptacle
|\highlight{\warningcolor}{Missing parameter: the furniture piece where the transfer happens}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?receptacle1)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?receptacle2)
    |\highlight{\warningcolor}{Incorrect precondition: connected is irrelevant to the action}|
    (connected ?receptacle1 ?receptacle2)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?food ?receptacle1)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?receptacle2)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (robot-holding ?irrelevantObject - householdObjects))
    |\highlight{\warningcolor}{Missing precondition: robot should hold nothing in its gripper}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle1 should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle2 should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle1 should be in/on furnitureAppliance}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle1 should be in/on furnitureAppliance}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle2 should be opened if it is openable}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle2 should be opened if it is openable}|
    |\highlight{\warningcolor}{Missing precondition: the furniture piece should have an open and flat surface}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?food ?receptacle1))
    (not (robot-holding ?food))
    |\highlight{\warningcolor}{Incorrect effect: ?irrelevantObject not a parameter}|
    (robot-holding ?irrelevantObject)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (put-on ?food ?receptacle2)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?food_1 - householdObject: the food to be transferred
|\highlight{\warningcolor}{Incorrect parameter: receptacle should be a householdObject}|
2. ?receptacle_1 - furnitureAppliance: the receptacle from which the food is transferred
|\highlight{\warningcolor}{Incorrect parameter: receptacle should be a householdObject}|
3. ?receptacle_2 - furnitureAppliance: the receptacle to which the food is transferred
|\highlight{\warningcolor}{Missing parameter: furnitureAppliance where the transfer happens}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?receptacle_1)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (robot-at ?receptacle_2)
    |\highlight{\warningcolor}{Incorrect precondition: connected is irrelevant to the action}|
    (connected ?receptacle_1 ?receptacle_2)
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?food_1 ?receptacle_1)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?receptacle_1)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?receptacle_2)
    |\highlight{\warningcolor}{Inaccurate precondition}|
    (openable ?receptacle_1)
    |\highlight{\warningcolor}{Inaccurate precondition: ?receptacle1 should be opened if it is openable}|
    (open ?receptacle_1)
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Incorrect precondition: ?food need not be pickupable}|
    (pickupable ?food_1)    
    |\highlight{\warningcolor}{Missing precondition: ?receptacle1 should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle2 should be a small receptacle}|
    |\highlight{\warningcolor}{Missing precondition: ?receptacle2 should be opened if it is openable}|
    |\highlight{\warningcolor}{Missing precondition: the furniture piece should have an open and flat surface}|
)


Effects:
(and
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (not (on ?food_1 ?receptacle_1))
    |\highlight{\warningcolor}{Incorrect effect: ?receptacle1 will not get clean}|
    (not (dirty ?receptacle_1))
    |\highlight{\minorcolor}{Irrelevant effect}|
    (not (robot-holding ?food_1))
    |\highlight{\warningcolor}{Incorrect use of the predicate}|
    (on ?food_1 ?receptacle_2)
    (dirty ?receptacle_2)
)

==> results/household_gpt35_pddl/unstack.tex <==
Parameters:
1. ?object_1 - householdObject: the object to be unstacked
|\highlight{\warningcolor}{Missing parameter: ?object\_2}|
|\highlight{\warningcolor}{Missing parameter: ?f1, the furniture piece where stacking happens}|

Preconditions:
(and
    (robot-at ?f1)
    |\highlight{\warningcolor}{Irrelevant precondition and syntax error}|
    (reachable ?f1 ?f2)
    (object-stacked-on ?object_1 ?object_2)
    (object-pickupable ?object_1)
    (object-pickupable ?object_2)
    (object-on ?object_2 ?f2)
    |\highlight{\warningcolor}{Inaccurate precondition}|
    (not (robot-holding ?o))
    |\highlight{\warningcolor}{Syntax error}|
    (not (object-in ?object_1 ?smallContainer))
    |\highlight{\warningcolor}{Syntax error}|
    (not (object-in ?object_2 ?smallContainer))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (furniture-openable ?object_2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (furniture-open ?object_2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (object-toggleable ?object_2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (object-sliceable ?object_2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (object-on-cutting-board ?object_2 ?f2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (cutting-board-closed ?f2))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (object-washed ?object_2))
)

Effects:
(and
    (not (object-stacked-on ?object_1 ?object_2))
    |\highlight{\warningcolor}{Unknown parameter}|
    (not (object-on ?object_1 ?f2))
    (robot-holding ?object_1)
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (object-pickupable ?object_1))
    (not (object-stacked ?object_1))
    |\highlight{\warningcolor}{Missing effect: ?object\_2 is clear}|
)

==> results/household_gpt35_pddl/vacuum.tex <==
Parameters:
1. ?x - householdObject: the handheld vacuum cleaner to use
2. ?y - furnitureAppliance: the carpet to vacuum

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x is held by robot}|
    (on ?x ?y)
    (robot-holding ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    |\highlight{\warningcolor}{Missing precondition: ?x is a vacuum}|
    |\highlight{\warningcolor}{Missing precondition: ?y is a carpet}|
)

Effects:
(and
    (not (on ?x ?y))
    (robot-holding ?x)
    (cleaned ?y)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the handheld vacuum cleaner to use
2. ?y - furnitureAppliance: the carpet to vacuum

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    (robot-holding ?x)
    (turned-on ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?x is held by robot}|
    (on ?x ?y)
    (pickupable ?x)
    (robot-holding-something)
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be clean}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Missing precondition: ?x is a vacuum}|
    |\highlight{\warningcolor}{Missing precondition: ?y is a carpet}|
    |\highlight{\warningcolor}{Missing precondition: the dust bin of ?x should be empty}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?x is held by robot}|
    (not (robot-holding ?x))
    |\highlight{\warningcolor}{Incorrect effect: ?y is cleaned}|
    (dirty ?y)
    |\highlight{\warningcolor}{Missing precondition: the dust bin of ?x should be full}|
)

==> results/household_gpt35_pddl/wash.tex <==
Parameters:
1. ?x - householdObject: the object to wash
2. ?y - furnitureAppliance: the sink or basin to use for washing

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (connected ?y ?x)
    (on ?x ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (open ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?z is not a parameter}|
    (not (robot-holding ?z))
    |\highlight{\warningcolor}{Incorrect precondition: ?z is not a parameter}|
    (not (smallAppliance ?z))
    |\highlight{\warningcolor}{Missing precondition: ?y should be a sink or basin}|
    |\highlight{\warningcolor}{Missing precondition: ?x is held by robot }|
)

Effects:
(and
    (not (on ?x ?y))
    (robot-holding ?x)
    |\highlight{\minorcolor}{Irrelevant effect}|
    (not (on-table ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (open ?y))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (cleaned ?y))
    |\highlight{\warningcolor}{Missing effect: ?x is cleaned}|
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - householdObject: the object to wash
|\highlight{\warningcolor}{Missing parameter: ?z, should be a sink basin}|

Preconditions:
(and
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (robot-at ?y - furnitureAppliance)
    |\highlight{\warningcolor}{Invalid use of the predicate}|
    (connected ?y ?z - furnitureAppliance)
    |\highlight{\warningcolor}{Incorrect precondition: ?x is held by robot}|
    (on ?x ?z)
    (robot-holding ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (cleanable ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?z)
    |\highlight{\warningcolor}{Incorrect precondition: ?x need not be clean}|
    (not (dirty ?x))
    |\highlight{\warningcolor}{Incorrect precondition: ?x is held by robot}|
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Missing precondition: ?z is a sink or basin}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect}|
    (cleaned ?z)
    |\highlight{\minorcolor}{Irrelevant effect}|
    (not (on ?x ?z))
    |\highlight{\warningcolor}{Incorrect effect: ?x is held by robot}|
    (not (robot-holding ?x))
    |\highlight{\minorcolor}{Irrelevant effect}|
    (robot-holding-something)
    |\highlight{\warningcolor}{Irrelevant effect}|
    (not (robot-holding knife))
    (not (dirty ?x))
    |\highlight{\warningcolor}{Incorrect effect: ?x is held by robot}|
    (on ?x ?z)
)

==> results/household_gpt35_pddl/wipe.tex <==
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to wipe and clean
|\highlight{\warningcolor}{Invalid object type: should be householdObject}|
2. ?y - householdObject: the cloth to use for wiping and cleaning

Preconditions:
(and
    (robot-at ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?x)
    (robot-holding ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?y is a cloth}|
    (not (turned-on ?y))
    |\highlight{\warningcolor}{Incorrect precondition: ?y is a cloth}|
    (not (turned-off ?y))
    |\highlight{\warningcolor}{Incorrect precondition: ?z is not a parameter}|
    (not (robot-holding ?z)) ; the robot is not holding any other irrelevant objects
    |\highlight{\warningcolor}{Missing precondition: ?y should be a cloth}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect effect: ?y is held by robot}|
    (not (robot-holding ?y))
    (cleaned ?x)
)
-------------------------------------------
|\highlight{\inputcolor}{With additional information:}|
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to wipe and clean
2. ?y - householdObject: the cloth to use for wiping and cleaning

Preconditions:
(and
    (robot-at ?x)
    |\highlight{\warningcolor}{Incorrect precondition: connected is irrelevant}|
    (connected ?x ?y)
    (robot-holding ?y)
    (cleanable ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (on-table ?y)
    (not (dirty ?y))
    |\highlight{\warningcolor}{Incorrect precondition: ?y is held by robot}|
    (not (robot-holding-something))
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (robot-holding knife))
    |\highlight{\warningcolor}{Missing precondition: ?y is a cloth}|
)

Effects:
(and
    (cleaned ?x)
    (dirty ?y)
)

==> results/household_gpt4_correction/heat_pan.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?f - householdObject: the food to be heated
|\highlight{\warningcolor}{There is an inaccurate object type: a pan ?p can be viewed as a small receptacle}|
2. ?p - householdObject: the pan to be used for heating the food
3. ?s - furnitureAppliance: the stove burner on which the pan is placed

Preconditions:
(and
    (robot-at ?s)
    |\highlight{\warningcolor}{Syntax error: the second parameter of `object-on` should}|
    |\highlight{\warningcolor}{    be a furnitureAppliance, but a householdObject was given}|
    (object-on ?f ?p)
    (object-on ?p ?s)
    |\highlight{\warningcolor}{Incorrect precondition: ?f needs not be pickupable}|
    (pickupable ?f)
    (is-small-receptacle ?p)
    |\highlight{\warningcolor}{Incorrect precondition: a stove or burner ?s doesn't need to have a flat surface}|
    (flat-surface ?s)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Missing precondition: ?p has to be a pan}|
    |\highlight{\warningcolor}{Missing precondition: ?s has to be a stove burner}|
)

Effects:
(and
    (not (pickupable ?f))
    (food-heated-pan ?f)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There are some errors in the PDDL model:
1. There is an inaccurate object type, a pan ?p can be viewed as a small receptacle
2. There is a syntax error: the second parameter of `object-on` should be a furnitureAppliance, but a householdObject was given. Please use the correct predicate or devise new one(s) if needed
3. Incorrect precondition: ?f needs not be pickupable
4. There is a missing precondition: ?p has to be a pan
5. There is a missing precondition: ?s has to be a stove burner
6. There is an incorrect precondition: a stove or burner ?s doesn't need to have a flat surface

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?f - householdObject: the food to be heated
2. ?p - smallReceptacle: the pan to be used for heating the food
3. ?s - furnitureAppliance: the stove burner on which the pan is placed

Preconditions:
(and
    (robot-at ?s)
    (object-in ?f ?p)
    (object-on ?p ?s)
    (pan ?p)
    (stove-burner ?s)
    (robot-hand-empty)
)

Effects:
(and
    (not (pickupable ?f))
    (food-heated-pan ?f)
)

New Predicates:
1. (pan ?x - smallReceptacle): true if the small receptacle ?x is a pan
2. (stove-burner ?x - furnitureAppliance): true if the furniture or appliance ?x is a stove burner
3. (object-in ?x - householdObject ?y - smallReceptacle): true if the object ?x is in the small receptacle ?y
----------------------------------------
|\highlight{\inputcolor}{Automated corrective feedback:}|
The following predicate(s) have the same name(s) as existing predicate(s):
1. (object-in ?x - householdObject ?y - smallReceptacle), true if the object ?x is in the small receptacle ?y; existing predicate with the same name: (object-in ?x - householdObject ?z - smallReceptacle), true if the object ?x is in the small receptacle ?z

You should reuse existing predicates whenever possible. If you are reusing existing predicate(s), you shouldn't list them under 'New Predicates'. If existing predicates are not enough and you are devising new predicate(s), please use names that are different from existing ones.

Please revise the PDDL model to fix this error.

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?f - householdObject: the food to be heated
2. ?p - smallReceptacle: the pan to be used for heating the food
3. ?s - furnitureAppliance: the stove burner on which the pan is placed

Preconditions:
(and
    (robot-at ?s)
    (object-in ?f ?p)
    (object-on ?p ?s)
    (pan ?p)
    (stove-burner ?s)
    (robot-hand-empty)
)

Effects:
(and
    (not (pickupable ?f))
    (food-heated-pan ?f)
)

New Predicates:
1. (pan ?x - smallReceptacle): true if the small receptacle ?x is a pan
2. (stove-burner ?x - furnitureAppliance): true if the furniture or appliance ?x is a stove burner

==> results/household_gpt4_correction/slice.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?x - householdObject: the object to slice
2. ?k - householdObject: the knife to use for slicing
3. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
|\highlight{\warningcolor}{Incorrect object type, a cutting board should be viewed as}|
|\highlight{\warningcolor}{    a small receptacle as mentioned in the prompt}|
4. ?z - householdObject: the cutting board on which the object is placed

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be on the cutting board not directly on the furniture ?y}|
    (object-on ?x ?y)
    (object-on ?z ?y)
    (robot-holding ?k)
    (sliceable ?x)
    (cutting-board ?z)
    (knife ?k)
    (flat-surface ?y)
    (object-whole ?x)
)

Effects:
(and
    (not (object-whole ?x))
    (object-sliced ?x)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There are some errors in the PDDL model:
1. There is an incorrect object type: a cutting board should be viewed as a small receptacle as mentioned in the prompt
2. There is an incorrect precondition: ?x should be on the cutting board not directly on the furniture ?y

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?x - householdObject: the object to slice
2. ?k - householdObject: the knife to use for slicing
3. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
4. ?z - smallReceptacle: the cutting board on which the object is placed

Preconditions:
(and
    (robot-at ?y)
    (object-in ?x ?z)
    (object-on ?z ?y)
    (robot-holding ?k)
    (sliceable ?x)
    (cutting-board ?z)
    (knife ?k)
    (flat-surface ?y)
    (object-whole ?x)
)

Effects:
(and
    (not (object-whole ?x))
    (object-sliced ?x)
)

New Predicates:
No newly defined predicate

==> results/household_gpt4_pddl/close.tex <==
Parameters:
1. ?y - furnitureAppliance: the furniture or appliance to close

Preconditions:
(and
    (robot-at ?y)
    (openable ?y)
    (opened ?y)
    (robot-hand-empty)
)

Effects:
(and
    (not (opened ?y))
    (closed ?y)
)

==> results/household_gpt4_pddl/close_small.tex <==
Parameters:
1. ?x - smallReceptacle: the small receptacle to close
2. ?y - furnitureAppliance: the furniture or appliance on which the small receptacle is placed

Preconditions:
(and
    (robot-at ?y)
    (object-on ?x ?y)
    (openable-receptacle ?x)
    (opened-receptacle ?x)
    (flat-surface ?y)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Inaccurate precondition: "?x is not stacked on other objects" should}|
    |\highlight{\warningcolor}{    only apply if ?x is a stackable object}|
    (not (object-stacked ?x))
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked on top of ?x}|
)

Effects:
(and
    (not (opened-receptacle ?x))
    (closed-receptacle ?x)
)

==> results/household_gpt4_pddl/empty_vacuum.tex <==
Parameters:
1. ?v - householdObject: the vacuum cleaner with a full dust bin
2. ?t - furnitureAppliance: the trash can where the dust will be dumped

Preconditions:
(and
    (robot-at ?t)
    (robot-holding ?v)
    (dustbin-full ?v)
    (pickupable ?v)
    |\highlight{\warningcolor}{Inaccurate precondition: ?t should be open only if it is openable}|
    (openable ?t)
    (opened ?t)
    |\highlight{\warningcolor}{Missing precondition: ?t should be a trash can}|
    |\highlight{\warningcolor}{Missing precondition: ?v should be a vacuum cleaner}|
)

Effects:
(and
    (not (dustbin-full ?v))
)

==> results/household_gpt4_pddl/goto.tex <==
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance the robot is currently at
2. ?y - furnitureAppliance: the furniture or appliance the robot wants to navigate to

Preconditions:
(and
    (robot-at ?x)
    (not (= ?x ?y))
)

Effects:
(and
    (not (robot-at ?x))
    (robot-at ?y)
)

==> results/household_gpt4_pddl/heat_microwave.tex <==
Parameters:
1. ?x - householdObject: the food to heat up
2. ?y - furnitureAppliance: the microwave to use
3. ?z - smallReceptacle: the small receptacle containing the food

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: the object should be in the receptacle not directly in the microwave}|
    (object-on ?x ?y)
    (object-in ?x ?z)
    (is-small-receptacle ?z)
    (object-on ?z ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x needs not be pickupable}|
    (pickupable ?x)
    (closed ?y)
    (not (food-heated ?x))
    |\highlight{\warningcolor}{Missing precondition: ?y should be a microwave}|
)

Effects:
(and
    (not (pickupable ?x))
    (food-heated ?x)
)

==> results/household_gpt4_pddl/heat_pan.tex <==
Parameters:
1. ?f - householdObject: the food to be heated
|\highlight{\warningcolor}{Inaccurate object type, a pan ?p can be viewed as a small receptacle}|
2. ?p - householdObject: the pan to be used for heating the food
3. ?s - furnitureAppliance: the stove burner on which the pan is placed

Preconditions:
(and
    (robot-at ?s)
    |\highlight{\warningcolor}{Syntax error: the second parameter of `object-on` should}|
    |\highlight{\warningcolor}{    be a furnitureAppliance, but a householdObject was given}|
    (object-on ?f ?p)
    (object-on ?p ?s)
    |\highlight{\warningcolor}{Incorrect precondition: ?f needs not be pickupable}|
    (pickupable ?f)
    (is-small-receptacle ?p)
    |\highlight{\warningcolor}{Incorrect precondition: a stove or burner ?s doesn't need to have a flat surface}|
    (flat-surface ?s)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Missing precondition: ?p has to be a pan}|
    |\highlight{\warningcolor}{Missing precondition: ?s has to be a stove burner}|
)

Effects:
(and
    (not (pickupable ?f))
    (food-heated-pan ?f)
)

==> results/household_gpt4_pddl/mash.tex <==
Parameters:
|\highlight{\warningcolor}{Incorrect object type: a blender ?b should be a smallReceptacle}|
1. ?b - householdObject: the blender to be used for mashing the food
2. ?f - householdObject: the food to be mashed
3. ?y - furnitureAppliance: the furniture or appliance where the blender is located

Preconditions:
(and
    (robot-at ?y)
    (object-on ?b ?y)
    |\highlight{\warningcolor}{Incorrect precondition: the food to mash should be in the blender ?b}|
    |\highlight{\warningcolor}{    rather than directly on the furniture piece ?y}|
    (object-on ?f ?y)
    (object-in ?f ?b)
    (object-sliced ?f)
    (is-small-receptacle ?b)
    |\highlight{\warningcolor}{Incorrect precondition: as mentioned in the prompt, the blender}|
    |\highlight{\warningcolor}{    should be turned off at the beginning}|
    (appliance-on ?b)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Missing precondition: ?b should be a blender}|
)

Effects:
(and
    (not (appliance-on ?b))
    (object-mashed ?f)
    |\highlight{\warningcolor}{Missing effect: ?f is no longer pickupable}|
)

==> results/household_gpt4_pddl/open.tex <==
Parameters:
1. ?y - furnitureAppliance: the furniture or appliance to be opened

Preconditions:
(and
    (robot-at ?y)
    (openable ?y)
    (closed ?y)
    (robot-hand-empty)
)

Effects:
(and
    (not (closed ?y))
    (opened ?y)
)

==> results/household_gpt4_pddl/open_small.tex <==
Parameters:
1. ?x - smallReceptacle: the small receptacle to be opened
2. ?y - furnitureAppliance: the furniture or appliance on which the small receptacle is placed

Preconditions:
(and
    (robot-at ?y)
    (object-on ?x ?y)
    (openable-receptacle ?x)
    (flat-surface ?y)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Inaccurate precondition: should only apply if ?x is stackable}|
    (not (object-stacked ?x))
    (closed-receptacle ?x)
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked on top of ?x}|
)

Effects:
(and
    (not (closed-receptacle ?x))
    (opened-receptacle ?x)
)

==> results/household_gpt4_pddl/pickup.tex <==
Parameters:
1. ?x - householdObject: the object to pick up
2. ?y - furnitureAppliance: the furniture or appliance where the object is located

Preconditions:
(and
    (robot-at ?y)
    (object-on ?x ?y)
    (pickupable ?x)
    |\highlight{\warningcolor}{Inaccurate precondition: "?x is not stacked on top of other object" should}|
    |\highlight{\warningcolor}{    only apply when ?x is a stackable object}|
    (not (object-stacked ?x))
    (robot-hand-empty)
    (or
        (not (openable ?y))
        (opened ?y)
    )
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked on top of}|
    |\highlight{\warningcolor}{    ?x if ?x is a stackable object}|
)

Effects:
(and
    (not (object-on ?x ?y))
    (robot-holding ?x)
    (not (robot-hand-empty))
)

==> results/household_gpt4_pddl/pickup_from_small.tex <==
Parameters:
1. ?x - householdObject: the object to pick up
2. ?y - furnitureAppliance: the furniture or appliance where the object is located
3. ?z - smallReceptacle: the small receptacle containing the object

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: the object ?x is in the receptacle ?z}|
    |\highlight{\warningcolor}{    so ?x is not directly on the furniture or appliance ?y}|
    (object-on ?x ?y)
    (pickupable ?x)
    (object-in ?x ?z)
    (is-small-receptacle ?z)
    |\highlight{\warningcolor}{Inaccurate precondition: "?z is not stacked on other objects" should}|
    |\highlight{\warningcolor}{    only apply if ?z is a stackable object}|
    (not (object-stacked ?z))
    (flat-surface ?y)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Incorrect precondition: ?x can't be stacked inside a receptacle so the precondition `?x is not}|
    |\highlight{\warningcolor}{    under other household object` is unnecessary}|
    (object-clear ?x)
    |\highlight{\warningcolor}{Incorrect precondition: ?z can be an openable receptacle}|
    (not (openable-receptacle ?z))
    (or
        |\highlight{\warningcolor}{Syntax error, the first parameter of `openable` should}|
        |\highlight{\warningcolor}{    be a furnitureAppliance but here a smallReceptacle is given}|
        (not (openable ?z))
        (opened-receptacle ?z)
    )
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked on top of ?z if ?z is stackable}|
)

Effects:
(and
    (not (object-on ?x ?y))
    (not (object-in ?x ?z))
    (not (robot-hand-empty))
    (robot-holding ?x)
)

==> results/household_gpt4_pddl/predicates.tex <==
1. (robot-at ?x - furnitureAppliance): true if the robot is at the furniture or appliance ?x
2. (object-on ?x - householdObject ?y - furnitureAppliance): true if the object ?x is on or in the furniture or appliance ?y
3. (pickupable ?x - householdObject): true if the object ?x can be picked up by the robot
4. (object-stacked ?x - householdObject): true if the object ?x is stacked on top of other household items
5. (openable ?y - furnitureAppliance): true if the furniture or appliance ?y can be opened
6. (opened ?y - furnitureAppliance): true if the furniture or appliance ?y is opened
7. (robot-holding ?x - householdObject): true if the robot is holding the object ?x
8. (robot-hand-empty): true if the robot's gripper is empty
9. (object-clear ?x - householdObject): true if the object ?x is not under any another household object
10. (appliance-on ?x - householdObject): true if the small appliance ?x is switched on
11. (sliceable ?x - householdObject): true if the object ?x can be sliced
12. (cutting-board ?z - householdObject): true if the object ?z is a cutting board
13. (knife ?k - householdObject): true if the object ?k is a knife
14. (flat-surface ?y - furnitureAppliance): true if the furniture or appliance ?y has a flat surface for manipulation
15. (object-whole ?x - householdObject): true if the object ?x is whole and not sliced
16. (object-sliced ?x - householdObject): true if the object ?x has been sliced
17. (food-heated ?x - householdObject): true if the food ?x has been heated in the microwave
18. (food-heated-pan ?x - householdObject): true if the food ?x has been heated with a pan
19. (is-small-receptacle ?x - householdObject): true if the object ?x is a small receptacle like bowls, lunch boxes, plates, etc.
20. (object-in ?x - householdObject ?z - smallReceptacle): true if the object ?x is in the small receptacle ?z
21. (openable-receptacle ?x - smallReceptacle): true if the small receptacle ?x can be opened
22. (opened-receptacle ?x - smallReceptacle): true if the small receptacle ?x is opened
23. (object-mashed ?x - householdObject): true if the object ?x has been mashed in the blender
24. (washable ?x - householdObject): true if the object ?x can be washed
25. (object-washed ?x - householdObject): true if the object ?x has been washed
26. (object-dirty ?x - householdObject): true if the object ?x is dirty
27. (dustbin-full ?v - householdObject): true if the dust bin of the vacuum cleaner ?v is full
28. (carpet-clean ?c - furnitureAppliance): true if the carpet ?c is clean
29. (closed ?y - furnitureAppliance): true if the furniture or appliance ?y is closed
30. (closed-receptacle ?x - smallReceptacle): true if the small receptacle ?x is closed
31. (furniture-cleaned ?x - furnitureAppliance): true if the furniture or appliance ?x has been wiped and cleaned

==> results/household_gpt4_pddl/prompt_example.tex <==
|\highlight{\commentcolor}{Instructions for the PDDL generation task}|
You are defining the preconditions and effects (represented in PDDL format) of an AI agent's actions. Information about the AI agent will be provided in the domain description. Note that individual conditions in preconditions and effects should be listed separately. For example, “object_1 is washed and heated” should be considered as two separate conditions “object_1 is washed” and “object_1 is heated”. Also, in PDDL, two predicates cannot have the same name even if they have different parameters. Each predicate in PDDL must have a unique name, and its parameters must be explicitly defined in the predicate definition. It is recommended to define predicate names in an intuitive and readable way.
|\highlight{\commentcolor}{One or two examples from other domains for illustrating the input and output formats}|
Here are two examples from the classical BlocksWorld domain for demonstrating the output format.

Domain information: BlocksWorld is a planning domain in artificial intelligence. The AI agent here is a mechanical robot arm that can pick and place the blocks. Only one block may be moved at a time: it may either be placed on the table or placed atop another block. Because of this, any blocks that are, at a given time, under another block cannot be moved. There is only one type of object in this domain, and that is the block.

Example 1
Action: This action enables the robot to put a block onto the table. For example, the robot puts block_1 onto the table.

You can create and define new predicates, but you may also reuse the following predicates:
No predicate has been defined yet

Parameters:
1. ?x - block: the block to put down

Preconditions:
```
(and
    (robot-holding ?x)
)
```

Effects:
```
(and
    (not (robot-holding ?x))
    (block-clear ?x)
    (robot-hand-empty)
    (block-on-table ?x)
)
```

New Predicates:
1. (robot-holding ?x - block): true if the robot arm is holding the block ?x
2. (block-clear ?x - block): true if the block ?x is not under any another block
3. (robot-hand-empty): true if the robot arm is not holding any block
4. (block-on-table ?x - block): true if the block ?x is placed on the table


Example 2
Action: This action enables the robot to pick up a block on the table.

You can create and define new predicates, but you may also reuse the following predicates:
1. (robot-holding ?x - block): true if the robot arm is holding the block ?x
2. (block-clear ?x - block): true if the block ?x is not under any another block
3. (robot-hand-empty): true if the robot arm is not holding any block
4. (block-on-table ?x - block): true if the block ?x is placed on the table

Parameters:
1. ?x - block: the block to pick up

Preconditions:
```
(and
    (block-clear ?x)
    (block-on-table ?x)
    (robot-hand-empty)
)
```

Effects:
```
(and
    (not (block-on-table ?x))
    (not (block-clear ?x))
    (not (robot-hand-empty))
    (robot-holding ?x)
)
```

New Predicates:
No newly defined predicate


Here is the task.
|\highlight{\commentcolor}{A natural language description of the domain}|
Domain information: The AI agent here is a household robot that can navigate to various large and normally immovable furniture pieces or appliances in the house to carry out household tasks. Note that the robot has only one gripper, so (a) it can only hold one object; (b) it shouldn't hold any other irrelevant objects in its gripper while performing some manipulation tasks (e.g., opening a drawer or closing a window); (c) operations on small household items should be carried out on furniture with a flat surface to get enough space for manipulation. There are three types of objects in this domain: robot, furnitureAppliance, and householdObject. The object type furnitureAppliance covers large and normally immovable furniture pieces or appliances, such as stove burners, side tables, dining tables, drawer, cabinets, or microwaves. The object type householdObject covers all other small household items, such as handheld vacuum cleaners, cloth, apples, bananas, and small receptacles like bowls and lunch boxes. In this domain, the locations of the robot and small household items (e.g., apples, oranges, bowls, lunch boxes or lamps) are determined by large and normally immovable furniture pieces or appliances.
|\highlight{\commentcolor}{A natural language description of the action}|
Action: This action enables the robot to close a small receptacle receptacle_1 that is openable (e.g. small storage boxes or lunch boxes with lids). For example, the robot closes lunch_box_2, or the robot closes storage_box_1.
|\highlight{\commentcolor}{The dynamically updated list of predicates}|
You can create and define new predicates, but you may also reuse the following predicates:
1. (robot-at ?x - furnitureAppliance): true if the robot is at the furniture or appliance ?x
2. (object-on ?x - householdObject ?y - furnitureAppliance): true if the object ?x is on or in the furniture or appliance ?y
3. (pickupable ?x - householdObject): true if the object ?x can be picked up by the robot
4. (closed-receptacle ?x - smallReceptacle): true if the small receptacle ?x is closed
...

Parameters:

==> results/household_gpt4_pddl/put.tex <==
Parameters:
1. ?x - householdObject: the object to put in/on the furniture or appliance
2. ?y - furnitureAppliance: the furniture or appliance to put the object in/on

Preconditions:
(and
    (robot-at ?y)
    (robot-holding ?x)
    (pickupable ?x)
    |\highlight{\warningcolor}{Unnecessary precondition "no other object stacked on object ?x"}|
    (object-clear ?x)
    (or
        (not (openable ?y))
        (opened ?y)
    )
)

Effects:
(and
    (not (robot-holding ?x))
    (robot-hand-empty)
    (object-on ?x ?y)
    |\highlight{\warningcolor}{Syntax error, there is an illegal keyword "if"}|
    (if (openable ?y) (closed ?y))
)

==> results/household_gpt4_pddl/put_into_small.tex <==
Parameters:
1. ?x - householdObject: the object to put into/onto the small receptacle
2. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
3. ?z - smallReceptacle: the small receptacle to put the object into/onto

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Inaccurate precondition: object ?x can't be on the furnitureAppliance ?y}|
    |\highlight{\warningcolor}{    when ?x is held by the robot}|
    (object-on ?x ?y)
    (pickupable ?x)
    |\highlight{\warningcolor}{Inaccurate precondition: this should only apply if ?z is stackable}|
    (not (object-stacked ?z))
    (flat-surface ?y)
    (robot-holding ?x)
    (is-small-receptacle ?z)
    (object-on ?z ?y)
    |\highlight{\warningcolor}{Inaccurate precondition:  this should only apply if ?z is stackable}|
    (object-clear ?z)
    |\highlight{\minorcolor}{Unnecessary precondition: the robot holding the object ?x already}|
    |\highlight{\minorcolor}{    implies ?x is not in the receptacle ?z}|
    (not (object-in ?x ?z))
    (or
        (not (openable-receptacle ?z))
        (opened-receptacle ?z)
    )
)

Effects:
(and
    (not (robot-holding ?x))
    (not (object-on ?x ?y))
    (robot-hand-empty)
    (object-in ?x ?z)
)

==> results/household_gpt4_pddl/slice.tex <==
Parameters:
1. ?x - householdObject: the object to slice
2. ?k - householdObject: the knife to use for slicing
3. ?y - furnitureAppliance: the furniture or appliance with a flat surface for manipulation
|\highlight{\warningcolor}{Incorrect object type, a cutting board should be viewed as}|
|\highlight{\warningcolor}{    a small receptacle as mentioned in the prompt}|
4. ?z - householdObject: the cutting board on which the object is placed

Preconditions:
(and
    (robot-at ?y)
    |\highlight{\warningcolor}{Incorrect precondition: ?x should be on the cutting board not directly on the furniture ?y}|
    (object-on ?x ?y)
    (object-on ?z ?y)
    (robot-holding ?k)
    (sliceable ?x)
    (cutting-board ?z)
    (knife ?k)
    (flat-surface ?y)
    (object-whole ?x)
)

Effects:
(and
    (not (object-whole ?x))
    (object-sliced ?x)
)

==> results/household_gpt4_pddl/stack.tex <==
Parameters:
1. ?x - householdObject: the object to stack on top of another object
2. ?y - householdObject: the object on which ?x will be stacked
3. ?z - furnitureAppliance: the furniture or appliance on which both objects are placed

Preconditions:
(and
    (robot-holding ?x)
    (object-on ?y ?z)
    (object-clear ?y)
    (flat-surface ?z)
    |\highlight{\warningcolor}{Incorrect precondition: should be stackable}|
    (pickupable ?x)
    |\highlight{\warningcolor}{Incorrect precondition: should be stackable}|
    (pickupable ?y)
    (robot-at ?z)
)

Effects:
(and
    (not (robot-holding ?x))
    (not (object-clear ?y))
    (robot-hand-empty)
    (object-on ?x ?z)
    (object-stacked ?x)
    |\highlight{\warningcolor}{Missing effect: object ?x should be stacked on top of object ?y}|
)

==> results/household_gpt4_pddl/toggle_off.tex <==
Parameters:
1. ?r - robot: the robot performing the action
2. ?o - householdObject: the small appliance to be toggled off
3. ?f - furnitureAppliance: the furniture or appliance where the small appliance is located

Preconditions:
(and
    (robot-at ?r ?f)
    (object-in-on-furniture ?o ?f)
    (robot-gripper-empty ?r)
    (appliance-on ?o)
)

Effects:
(and
    (not (appliance-on ?o))
)

==> results/household_gpt4_pddl/toggle_on.tex <==
Parameters:
1. ?x - householdObject: the small appliance to toggle on
2. ?y - furnitureAppliance: the furniture or appliance where the small appliance is located

Preconditions:
(and
    (robot-at ?y)
    (object-on ?x ?y)
    (robot-hand-empty)
    (not (appliance-on ?x))
    |\highlight{\warningcolor}{Missing precondition: the appliance to toggle should be a toggleable appliance}|
)

Effects:
(and
    (appliance-on ?x)
)

==> results/household_gpt4_pddl/transfer.tex <==
Parameters:
1. ?food - householdObject: the food to be transferred
2. ?receptacle1 - smallReceptacle: the small receptacle from which the food will be transferred
3. ?receptacle2 - smallReceptacle: the small receptacle to which the food will be transferred
4. ?furniture - furnitureAppliance: the furniture piece with a flat surface where the transfer will take place

Preconditions:
(and
    (robot-at ?furniture)
    (object-on ?receptacle1 ?furniture)
    (object-on ?receptacle2 ?furniture)
    (object-in ?food ?receptacle1)
    (is-small-receptacle ?receptacle1)
    (is-small-receptacle ?receptacle2)
    (flat-surface ?furniture)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Inaccurate precondition: "?receptacle1 is not stacked on other objects" should}|
    |\highlight{\warningcolor}{    only apply if ?receptacle1 is a stackable object}|
    (not (object-stacked ?receptacle1))
    |\highlight{\warningcolor}{Inaccurate precondition: "?receptacle2 is not stacked on other objects" should}|
    |\highlight{\warningcolor}{    only apply if ?receptacle2 is a stackable object}|
    (not (object-stacked ?receptacle2))
    (or (not (openable-receptacle ?receptacle1)) (opened-receptacle ?receptacle1))
    (or (not (openable-receptacle ?receptacle2)) (opened-receptacle ?receptacle2))
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked}|
    |\highlight{\warningcolor}{    on top of ?receptacle1 if ?receptacle1 is stackable}|
    |\highlight{\warningcolor}{Missing precondition: there should be no other object stacked}|
    |\highlight{\warningcolor}{    on top of ?receptacle2 if ?receptacle2 is stackable}|
)

Effects:
(and
    (not (object-in ?food ?receptacle1))
    (object-in ?food ?receptacle2)
)

==> results/household_gpt4_pddl/unstack.tex <==
Parameters:
1. ?x - householdObject: the object to unstack from another object
2. ?y - householdObject: the object that ?x is stacked on
3. ?z - furnitureAppliance: the furniture or appliance where the objects are stacked

Preconditions:
(and
    (robot-at ?z)
    (object-on ?x ?z)
    (object-on ?y ?z)
    (pickupable ?x)
    (object-stacked ?x)
    (object-clear ?x)
    (robot-hand-empty)
    |\highlight{\warningcolor}{Missing precondition: object ?x should be stacked on top of object ?y}|
)

Effects:
(and
    (not (object-on ?x ?z))
    (not (object-stacked ?x))
    |\highlight{\warningcolor}{Incorrect effect, this action shouldn't change whether or not object ?x}|
    |\highlight{\warningcolor}{    is under any another household object}|
    (not (object-clear ?x))
    (not (robot-hand-empty))
    (robot-holding ?x)
    (object-clear ?y)
    |\highlight{\warningcolor}{Missing effect: object ?x is no longer stacked on top of object ?y}|
)

==> results/household_gpt4_pddl/vacuum.tex <==
Parameters:
1. ?v - householdObject: the handheld vacuum cleaner to use
2. ?c - furnitureAppliance: the carpet to vacuum

Preconditions:
(and
    (robot-holding ?v)
    (robot-at ?c)
    (pickupable ?v)
    (not (dustbin-full ?v))
    (not (carpet-clean ?c))
    |\highlight{\warningcolor}{Missing precondition: ?v should be a handheld vacuum cleaner}|
    |\highlight{\warningcolor}{Missing precondition: ?c should be a carpet}|
)

Effects:
(and
    (carpet-clean ?c)
    (dustbin-full ?v)
)

==> results/household_gpt4_pddl/wash.tex <==
Parameters:
1. ?x - householdObject: the object to be washed
2. ?y - furnitureAppliance: the sink or basin where the object will be washed

Preconditions:
(and
    (robot-at ?y)
    (washable ?x)
    (robot-holding ?x)
    |\highlight{\warningcolor}{Missing precondition: ?y should be a sink or basin}|
)

Effects:
(and
    (not (object-dirty ?x))
    (object-washed ?x)
)

==> results/household_gpt4_pddl/wipe.tex <==
Parameters:
1. ?x - furnitureAppliance: the furniture or appliance to be wiped and cleaned
2. ?c - householdObject: the cloth to be used for wiping and cleaning

Preconditions:
(and
    (robot-at ?x)
    (robot-holding ?c)
    (washable ?c)
    (object-washed ?c)
    |\highlight{\warningcolor}{Incorrect precondition: ?x doesn't need to have a flat surface}|
    (flat-surface ?x)
    |\highlight{\warningcolor}{Missing precondition: ?c should be a cloth}|
)

Effects:
(and
    (not (object-washed ?c))
    (object-dirty ?c)
    (furniture-cleaned ?x)
)

==> results/llm_planner/action_translation_prompt.tex <==
Your task is to translate free-form action description to its corresponding structural format based on its semantic meaning. The structural output format is given in the example output of each candidate action. You should strictly follow the structural output format. When there is missing information in the free-form action description, you should output "Not able to translate due to missing information".

Here are 4 examples.
Example 1:
Action description: put bowl_1 with sliced orange_1 in/on dining_table_1
Candidate actions:
1. put an object on or in a furniture piece or an appliance, example output: "put apple_1 in/on side_table_1"
2. puts an object onto or into a small receptacle, example output: "put apple_1 in/on plate_1 at countertop_1"
Translated action: put bowl_1 in/on side_table_1

Example 2:
Action description: put sliced orange_1 in/on bowl_1 at drawer_1
Candidate actions:
1. put an object on or in a furniture piece or an appliance, example output: "put apple_1 in/on side_table_1"
2. puts an object onto or into a small receptacle, example output: "put apple_1 in/on plate_1 at countertop_1"
Translated action: put orange_1 in/on bowl_1 at drawer_1

Example 3:
Action description: pick up bowl_1 with sliced orange_1 in/on countertop_1
Candidate actions:
1. pick up an object on or in a furniture piece or an appliance, example output: "pick up apple_1 in/on side_table_1"
2. pick up an object on or in a small receptacle, example output: "pick up apple_1 in/on plate_1 at countertop_1"
Translated action: pick up bowl_1 in/on countertop_1

Example 4:
Action description: put mashed apple_1 in/on plate_1
Candidate actions:
1. put an object on or in a furniture piece or an appliance, example output: "put apple_1 in/on side_table_1"
2. puts an object onto or into a small receptacle, example output: "put apple_1 in/on plate_1 at countertop_1"
Translated action: Not able to translate due to missing information
            
Here is the task.

==> results/llm_planner/goal_to_pddl_prompt.tex <==
Your task is to translate natural language instructions to planning goals in planning domain definition language (PDDL). You should only use the given predicates to express the goal specification.

Here is an example from the classical BlocksWorld domain for demonstrating the output format.

Domain information: BlocksWorld is a planning domain in artificial intelligence. The AI agent here is a mechanical robot arm that can pick and place the blocks. Only one block may be moved at a time: it may either be placed on the table or placed atop another block. Because of this, any blocks that are, at a given time, under another block cannot be moved. There is only one type of object in this domain, and that is the block.

The domain has the following objects: block_1 (type: block), block_2 (type: block), block_3 (type: block), block_4 (type: block), block_5 (type: block).

Predicates:
1. (robot-holding ?x - block): true if the robot arm is holding the block ?x
2. (block-clear ?x - block): true if the block ?x is not under any another block
3. (robot-hand-empty): true if the robot arm is not holding any block
4. (block-on-table ?x - block): true if the block ?x is placed on the table
5. (on ?x - block ?y - block): true if block ?x is on top of block ?y

Instruction: rearrange the blocks such that block_1 is on top of block_2, block_2 is on top of block_3, and block_5 is not on the table.

Goal in PDDL:
```
(:goal
    (and
        (on block_1 block_2)
        (on block_2 block_3)
        (not (block-on-table block_5))
    )
)
```


Here is the task.

Domain information: xxx.

==> results/llm_planner/pddl_to_nl_prompt.tex <==
Your task is to translate planning domain definition language (PDDL) to natural language.

Here is an example:

Predicates:
1. (robot-holding ?x - block): true if the robot arm is holding the block ?x
2. (block-clear ?x - block): true if the block ?x is not under any another block
3. (robot-hand-empty): true if the robot arm is not holding any block
4. (block-on-table ?x - block): true if the block ?x is placed on the table

Contextual information: N/A

PDDL:
```
(and
    (not (robot-holding x1))
    (block-clear x1)
    (robot-hand-empty)
    (block-on-table x1)
)
```

Translated PDDL:
(and
    The robot arm is not holding the block x1;
    The block x1 is not under any another block;
    The robot arm is not holding any block;
    The block x1 is placed on the table;
)


Here is the task:

==> results/logistics_action_description/drive_truck.tex <==
This action enables the agent to drive a truck from one location to another in a city. For example, drive a truck_1 from location_1 to location_2 in city_1.

==> results/logistics_action_description/fly_plane.tex <==
This action enables the agent to fly an airplane from one city's airport to another. The airports are locations in the city. For example, fly an airplane_1 from location_0 to location_1.

==> results/logistics_action_description/load_airplane.tex <==
This action enables the agent to load a package into an airplane. For example, load a package_1 into an airplane_1.

==> results/logistics_action_description/load_truck.tex <==
This action enables the agent to load a package into a truck. For example, load a package_1 into a truck_1.

==> results/logistics_action_description/unload_airplane.tex <==
This action enables the agent to unload a package from an airplane. For example, unload a package_1 from an airplane_1.

==> results/logistics_action_description/unload_truck.tex <==
This action enables the agent to unload a package from a truck. For example, unload a package_1 from a truck_1.

==> results/logistics_gpt35_correction/fly_plane.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?a - plane: the airplane to fly
2. ?from - location: the departure location (airport) in the origin city
3. ?to - location: the destination location (airport) in the destination city
4. ?c1 - city: the origin city
5. ?c2 - city: the destination city

Preconditions:
(and
    (plane-at ?a ?from)
    (location-in-city ?from ?c1)
    (location-in-city ?to ?c2)
    (not (= ?c1 ?c2))
    |\highlight{\warningcolor}{Missing precondition: ?from should be an airport}|
    |\highlight{\warningcolor}{Missing precondition: ?to should be an airport}|
)

Effects:
(and
    (not (plane-at ?a ?from))
    (plane-at ?a ?to)
    (move-packages-plane ?a ?from ?to)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There is an error in the PDDL model:
1. The current action model allows the plane to fly from any location to another location in a different city, but a plane can only land at airports

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-3.5-Turbo:}|
1. ?a - plane: the airplane to fly
2. ?from - location: the departure location (airport) in the origin city
3. ?to - location: the destination location (airport) in the destination city
4. ?c1 - city: the origin city
5. ?c2 - city: the destination city

Preconditions:
(and
    (plane-at ?a ?from)
    (location-in-city ?from ?c1)
    (location-in-city ?to ?c2)
    (not (= ?c1 ?c2))
    (airport ?to)
    |\highlight{\warningcolor}{Missing precondition: ?from should be an airport}|
)

Effects:
(and
    (not (plane-at ?a ?from))
    (plane-at ?a ?to)
    (move-packages-plane ?a ?from ?to)
)

New Predicates:
1. (airport ?l - location): true if the location ?l is an airport.

==> results/logistics_gpt35_pddl/fly_plane.tex <==
Parameters:
1. ?a - plane: the airplane to fly
2. ?c1 - city: the city to fly from
3. ?c2 - city: the city to fly to
4. ?l1 - location: the airport location in ?c1
5. ?l2 - location: the airport location in ?c2

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (at ?a ?l1)
    (in-city ?l1 ?c1)
    (in-city ?l2 ?c2)
    (not (= ?c1 ?c2))
    |\highlight{\warningcolor}{Missing precondition: ?l1 should be an airport}|
    |\highlight{\warningcolor}{Missing precondition: ?l2 should be an airport}|
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (not (at ?a ?l1))
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (at ?a ?l2)
)

==> results/logistics_gpt35_pddl/load_truck.tex <==
Parameters:
1. ?p - package: the package to load
2. ?t - truck: the truck to load the package into
|\highlight{\warningcolor}{Missing parameter: ?l, the current location of the truck}|
|\highlight{\warningcolor}{Missing parameter: ?c, the current city}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (at ?p ?l)
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (at ?t ?l)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (truck-empty ?t)
    (in-city ?l ?c)
)

Effects:
(and
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (not (at ?p ?l))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (truck-empty ?t))
    |\highlight{\warningcolor}{Incorrect predicate design}|
    (at ?p ?t)
)

==> results/logistics_gpt35_pddl/unload_truck.tex <==
Parameters:
1. ?p - package: the package to unload
2. ?t - truck: the truck to unload from
|\highlight{\warningcolor}{Missing parameter: ?l, the location of the truck}|

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error and incorrect predicate design}|
    (at ?t - truck ?l - location)
    |\highlight{\warningcolor}{Syntax error and incorrect predicate design}|
    (at ?p - package ?t - truck)
)

Effects:
(and
    |\highlight{\warningcolor}{Syntax error}|
    (at ?p - package ?l - location)
    |\highlight{\warningcolor}{Syntax error}|
    (not (at ?p - package ?t - truck))
    |\highlight{\warningcolor}{Syntax error and incorrect effect}|
    (not (truck-empty ?t - truck))
)

==> results/logistics_gpt4_correction/fly_plane.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?a - plane: the airplane to fly
2. ?from - location: the departure location (airport) in the origin city
3. ?to - location: the destination location (airport) in the destination city
4. ?c1 - city: the origin city
5. ?c2 - city: the destination city

Preconditions:
(and
    (plane-at ?a ?from)
    (location-in-city ?from ?c1)
    (location-in-city ?to ?c2)
    (not (= ?c1 ?c2))
    |\highlight{\warningcolor}{Missing precondition: ?from should be an airport}|
    |\highlight{\warningcolor}{Missing precondition: ?to should be an airport}|
)

Effects:
(and
    (not (plane-at ?a ?from))
    (plane-at ?a ?to)
    (move-packages-plane ?a ?from ?to)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There is an error in the PDDL model:
1. The current action model allows the plane to fly from any location to another location in a different city, but a plane can only land at airports

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?a - plane: the airplane to fly
2. ?from - location: the departure location (airport) in the origin city
3. ?to - location: the destination location (airport) in the destination city
4. ?c1 - city: the origin city
5. ?c2 - city: the destination city

Preconditions:
(and
    (plane-at ?a ?from)
    (location-in-city ?from ?c1)
    (location-in-city ?to ?c2)
    (not (= ?c1 ?c2))
    (airport ?from)
    (airport ?to)
)

Effects:
(and
    (not (plane-at ?a ?from))
    (plane-at ?a ?to)
    (move-packages-plane ?a ?from ?to)
)

New Predicates:
1. (airport ?l - location): true if the location ?l is an airport

==> results/logistics_gpt4_pddl/drive_truck.tex <==
Parameters:
1. ?t - truck: the truck to be driven
2. ?from - location: the starting location of the truck
3. ?to - location: the destination location of the truck
4. ?c - city: the city in which the truck is being driven

Preconditions:
(and
    (truck-at ?t ?from)
    (location-in-city ?from ?c)
    (location-in-city ?to ?c)
    (not (= ?from ?to))
)

Effects:
(and
    (not (truck-at ?t ?from))
    (truck-at ?t ?to)
    (move-packages ?t ?from ?to)
)

==> results/logistics_gpt4_pddl/fly_plane.tex <==
Parameters:
1. ?a - plane: the airplane to fly
2. ?from - location: the departure location (airport) in the origin city
3. ?to - location: the destination location (airport) in the destination city
4. ?c1 - city: the origin city
5. ?c2 - city: the destination city

Preconditions:
(and
    (plane-at ?a ?from)
    (location-in-city ?from ?c1)
    (location-in-city ?to ?c2)
    (not (= ?c1 ?c2))
    |\highlight{\warningcolor}{Missing precondition: ?from should be an airport}|
    |\highlight{\warningcolor}{Missing precondition: ?to should be an airport}|
)

Effects:
(and
    (not (plane-at ?a ?from))
    (plane-at ?a ?to)
    (move-packages-plane ?a ?from ?to)
)

==> results/logistics_gpt4_pddl/load_airplane.tex <==
Parameters:
1. ?p - package: the package to load into the airplane
2. ?a - plane: the airplane to load the package into
3. ?l - location: the location where the package and airplane are present

Preconditions:
(and
    (package-at ?p ?l)
    (plane-at ?a ?l)
    (not (package-in-plane ?p ?a))
)

Effects:
(and
    (not (package-at ?p ?l))
    (package-in-plane ?p ?a)
)

==> results/logistics_gpt4_pddl/load_truck.tex <==
Parameters:
1. ?p - package: the package to load
2. ?t - truck: the truck to load the package into
3. ?l - location: the location where the package and truck are

Preconditions:
(and
    (package-at ?p ?l)
    (truck-at ?t ?l)
)

Effects:
(and
    (not (package-at ?p ?l))
    (package-in-truck ?p ?t)
)

==> results/logistics_gpt4_pddl/predicates.tex <==
1. (package-at ?p - package ?l - location): true if the package ?p is at the location ?l
2. (truck-at ?t - truck ?l - location): true if the truck ?t is at the location ?l
3. (package-in-truck ?p - package ?t - truck): true if the package ?p is in the truck ?t
4. (plane-at ?a - plane ?l - location): true if the airplane ?a is at the location ?l
5. (location-in-city ?l - location ?c - city): true if the location ?l is in the city ?c
6. (package-in-plane ?p - package ?a - plane): true if the package ?p is in the airplane ?a
7. (move-packages ?t - truck ?from - location ?to - location): true if all packages in the truck ?t are moved from location ?from to location ?to. This predicate is used to represent the effect of moving all packages in the truck when the truck is driven from one location to another.
8. (move-packages-plane ?a - plane ?from - location ?to - location): true if all packages in the airplane ?a are moved from location ?from to location ?to. This predicate is used to represent the effect of moving all packages in the airplane when the airplane is flown from one location to another

==> results/logistics_gpt4_pddl/unload_airplane.tex <==
Parameters:
1. ?p - package: the package to unload
2. ?a - plane: the airplane from which the package will be unloaded
3. ?l - location: the location where the airplane is and the package will be unloaded

Preconditions:
(and
    (package-in-plane ?p ?a)
    (plane-at ?a ?l)
)

Effects:
(and
    (not (package-in-plane ?p ?a))
    (package-at ?p ?l)
)

==> results/logistics_gpt4_pddl/unload_truck.tex <==
Parameters:
1. ?p - package: the package to unload
2. ?t - truck: the truck from which the package will be unloaded
3. ?l - location: the location where the package will be unloaded

Preconditions:
(and
    (package-in-truck ?p ?t)
    (truck-at ?t ?l)
)

Effects:
(and
    (not (package-in-truck ?p ?t))
    (package-at ?p ?l)
)

==> results/tyreworld_action_description/close_container.tex <==
This action enables the robot to close a container. For example, the robot can close a boot.

==> results/tyreworld_action_description/fasten.tex <==
This action enables the robot to fasten a hub by installing a nut on it. For example, the robot can fasten hub_1 that has nut_1. Note that the robot needs to install a nut into the hub, but the robot is not required to fasten the nut in this operation. To safely perform this action, the hub needs to be jacked up.

==> results/tyreworld_action_description/fetch_from_container.tex <==
This action enables the robot to take an object from a container. For example, the robot can fetch jack from the boot or the robot can fetch wheel_1 from the boot.

==> results/tyreworld_action_description/inflate.tex <==
This action enables the robot to inflate a wheel. For example, the robot can inflate wheel_1. Note that you need to make sure the wheel is intact.

==> results/tyreworld_action_description/jack_down.tex <==
This action enables the robot to jack down a hub. For example, the robot can jack down hub_1.

==> results/tyreworld_action_description/jack_up.tex <==
This action enables the robot to jack up a hub. For example, the robot can jack up hub_1.

==> results/tyreworld_action_description/loosen_nut.tex <==
This action enables the robot to loosen a nut in a hub. For example, the robot can loosen nut_1 in hub_1. To safely perform this action, the hub needs to be on the ground (i.e., not jacked up).

==> results/tyreworld_action_description/open_container.tex <==
This action enables the robot to open a container. For example, the robot can open a boot.

==> results/tyreworld_action_description/predicates.tex <==
1. (container-closed ?c - container): true if the container ?c is closed
2. (container-open ?c - container): true if the container ?c is open
3. (object-in-container ?x - small_object ?c - container): true if the small_object ?x is inside the container ?c
4. (robot-holding ?x - small_object): true if the robot is holding the small_object ?x
5. (is-wrench ?x - small_object): true if the small_object ?x is a wrench
6. (is-nut ?x - small_object): true if the small_object ?x is a nut
7. (is-hub ?x - hub): true if the object ?x is a hub
8. (nut-in-hub ?n - nut ?h - hub): true if the nut ?n is in the hub ?h
9. (hub-on-ground ?h - hub): true if the hub ?h is on the ground (not jacked-up)
10. (nut-loose ?n - nut): true if the nut ?n is loosened
11. (is-jack ?x - small_object): true if the small_object ?x is a jack
12. (hub-jacked-up ?h - hub): true if the hub ?h is jacked up (not on the ground)
13. (hub-unfastened ?h - hub): true if the hub ?h is unfastened
14. (is-wheel ?x - small_object): true if the small_object ?x is a wheel
15. (wheel-on-hub ?w - wheel ?h - hub): true if the wheel ?w is on the hub ?h
16. (is-pump ?x - small_object): true if the small_object ?x is a pump
17. (wheel-intact ?w - wheel): true if the wheel ?w is intact
18. (wheel-deflated ?w - wheel): true if the wheel ?w is deflated
19. (wheel-inflated ?w - wheel): true if the wheel ?w is inflated

==> results/tyreworld_action_description/put_container.tex <==
This action enables the robot to put an object into a container. For example, the robot can put away jack into the boot or the robot can put away wheel_1 into the boot.

==> results/tyreworld_action_description/put_wheel.tex <==
This action enables the robot to put a wheel on an unfastened hub. For example, the robot can put wheel_1 on hub_1. Note that the hub needs to be unfastened in order to put on the wheel. To safely perform this action, the hub needs to be jacked up.

==> results/tyreworld_action_description/remove_wheel.tex <==
This action enables the robot to remove a wheel from a hub. For example, the robot can remove wheel_1 from hub_1. Note that the hub needs to be unfastened in order to remove the wheel. To safely perform this action, the hub needs to be jacked up.

==> results/tyreworld_action_description/tighten_nut.tex <==
This action enables the robot to tighten a nut in a hub. For example, the robot can tighten nut_1 in hub_1. To safely perform this action, the hub needs to be on the ground (i.e., not jacked up).

==> results/tyreworld_action_description/unfasten.tex <==
This action enables the robot to unfasten a hub and remove the nut on it. For example, the robot can unfasten hub_1 that has nut_1. At the end of this action, the hub should be unfastened, and the nut should be detached from the hub and held by the robot. To safely perform this action, the hub needs to be jacked up.

==> results/tyreworld_gpt35_pddl/close_container.tex <==
Parameters:
1. ?x - container: the container to close

Preconditions:
(and
    (container-open ?x)
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameter}|
    (robot-holding ?y)
    |\highlight{\warningcolor}{Incorrect precondition and syntax error}|
    (tool-type ?y "lid")
)

Effects:
(and
    (not (container-open ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (robot-holding ?y))
)

==> results/tyreworld_gpt35_pddl/fasten.tex <==
Parameters:
1. ?x - hub: the hub to fasten
|\highlight{\warningcolor}{Missing parameter: ?y, the nut in the hub}|

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (robot-holding ?w - tool)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (tool-type ?w "wrench")
    |\highlight{\warningcolor}{Syntax error and incorrect precondition}|
    (nut-in-hub ?n - nut ?x)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (nut-loosened ?n))
    (hub-jacked-up ?x)
    |\highlight{\warningcolor}{Missing precondition: robot is holding the nut}|
    |\highlight{\warningcolor}{Missing precondition: ?x is unfastened}|
)

Effects:
(and
    (nut-loosened ?n)
    |\highlight{\warningcolor}{Missing effect: ?x is in the hub ?y}|
    |\highlight{\warningcolor}{Missing effect: ?x is fastened}|
    |\highlight{\warningcolor}{Missing effect: ?y is loose}|

)

==> results/tyreworld_gpt35_pddl/fetch_from_container.tex <==
Parameters:
1. ?x - small_object: the object to fetch
2. ?y - container: the container from which to fetch the object

Preconditions:
(and
    (container-open ?y)
    (object-in-container ?x ?y)
)

Effects:
(and
    (not (object-in-container ?x ?y))
    (robot-holding ?x)
)

==> results/tyreworld_gpt35_pddl/inflate.tex <==
Parameters:
1. ?x - wheel: the wheel to inflate
|\highlight{\warningcolor}{Missing parameter: the pump to use}|

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error}|
    (robot-holding ?pump - tool)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?pump "pump")
    (wheel-intact ?x)
    (wheel-deflated ?x)
)

Effects:
(and
    (not (wheel-deflated ?x))
    (wheel-intact ?x)
)

==> results/tyreworld_gpt35_pddl/jack_down.tex <==
Parameters:
1. ?x - hub: the hub to jack down
|\highlight{\warningcolor}{Missing parameter: ?y, the jack to use}|

Preconditions:
(and
    (robot-holding ?y)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?y "jack")
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (container-open ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (object-in-container ?y ?z)
    (hub-jacked-up ?x)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (wheel-attached ?y ?x)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (wheel-intact ?y)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (not (wheel-deflated ?y))
)

Effects:
(and
    (not (hub-jacked-up ?x))
    |\highlight{\warningcolor}{Syntax error and incorrect effect}|
    (not (wheel-attached ?y ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (wheel-detached ?y)
    |\highlight{\warningcolor}{Incorrect effect}|
    (robot-holding ?y)
)

==> results/tyreworld_gpt35_pddl/jack_up.tex <==
Parameters:
1. ?x - hub: the hub to jack up
|\highlight{\warningcolor}{Missing parameter: the jack to use}|

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error}|
    (robot-holding ?w - tool)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?w "jack")
    |\highlight{\warningcolor}{Syntax error}|
    (container-open ?c - container)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (object-in-container ?w ?c)
    |\highlight{\warningcolor}{Syntax error}|
    (nut-in-hub ?n - nut ?x)
    |\highlight{\warningcolor}{Syntax error}|
    (robot-holding ?l - tool)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?l "lid")
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameters}|
    (object-in-container ?l ?c)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (wheel-attached ?whe - wheel ?x)
    |\highlight{\warningcolor}{Unknown parameter and irrelevant precondition}|
    (wheel-intact ?whe)
    |\highlight{\warningcolor}{Unknown parameter and irrelevant precondition}|
    (not (wheel-deflated ?whe))
    (not (hub-jacked-up ?x))
)

Effects:
(and
    (hub-jacked-up ?x)
    |\highlight{\warningcolor}{Unknown parameter and incorrect effect}|
    (not (wheel-attached ?whe - wheel ?x))
    |\highlight{\warningcolor}{Unknown parameter and incorrect effect}|
    (wheel-detached ?whe)
)

==> results/tyreworld_gpt35_pddl/loosen_nut.tex <==
Parameters:
1. ?x - nut: the nut to loosen
2. ?y - hub: the hub containing the nut
|\highlight{\warningcolor}{Missing parameter: ?z, the wrench}|

Preconditions:
(and
    (not (hub-jacked-up ?y))
    (robot-holding ?z)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?z wrench)
    (nut-in-hub ?x ?y)
    (not (nut-loosened ?x))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (wheel-detached ?w))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (wheel-attached ?w ?y)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (wheel-intact ?w)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (wheel-deflated ?w))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (object-in-container ?z ?c)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (container-open ?c)
)

Effects:
(and
    (nut-loosened ?x)
)

==> results/tyreworld_gpt35_pddl/open_container.tex <==
Parameters:
1. ?x - container: the container to open

Preconditions:
(and
    (not (container-open ?x))
    |\highlight{\warningcolor}{Incorrect precondition and unknown parameter}|
    (robot-holding ?y)
    |\highlight{\warningcolor}{Incorrect precondition and syntax error}|
    (tool-type ?y "key")
    |\highlight{\warningcolor}{Incorrect precondition and syntax error}|
    (not (hub-jacked-up ?z))
)

Effects:
(and
    (container-open ?x)
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (robot-holding ?y))
)

==> results/tyreworld_gpt35_pddl/put_container.tex <==
Parameters:
1. ?x - small_object: the object to put away
2. ?y - container: the container to put the object into

Preconditions:
(and
    (robot-holding ?x)
    (container-open ?y)
)

Effects:
(and
    (not (robot-holding ?x))
    (object-in-container ?x ?y)
)

==> results/tyreworld_gpt35_pddl/put_wheel.tex <==
Parameters:
1. ?wheel - wheel: the wheel to be attached
2. ?hub - hub: the hub to which the wheel is to be attached

Preconditions:
(and
    (robot-holding ?wheel)
    (hub-jacked-up ?hub)
    |\highlight{\warningcolor}{Unnecessary precondition}|
    (not (wheel-attached ?wheel ?hub))
    |\highlight{\warningcolor}{Unnecessary precondition}|
    (wheel-intact ?wheel)
    |\highlight{\warningcolor}{Unnecessary precondition}|
    (not (wheel-deflated ?wheel))
    |\highlight{\warningcolor}{Incorrect precondition}|
    (tool-type ?wrench - tool "wrench")
    |\highlight{\warningcolor}{Incorrect precondition}|
    (robot-holding ?wrench)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (nut-in-hub ?nut - nut ?hub)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (robot-holding ?nut)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (nut-loosened ?nut))
    |\highlight{\warningcolor}{Missing precondition: hub unfastened}|
)

Effects:
(and
    (not (robot-holding ?wheel))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (robot-holding ?wrench))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (robot-holding ?nut))
    (wheel-attached ?wheel ?hub)
    |\highlight{\warningcolor}{Incorrect effect}|
    (nut-loosened ?nut)
)

==> results/tyreworld_gpt35_pddl/remove_wheel.tex <==
Parameters:
1. ?wheel - wheel: the wheel to remove
2. ?hub - hub: the hub from which the wheel is to be removed

Preconditions:
(and
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (robot-holding ?wrench - tool)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (tool-type ?wrench wrench)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (nut-in-hub ?nut - nut ?hub)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (robot-holding ?nut - small_object)
    |\highlight{\warningcolor}{Syntax error}|
    (wheel-attached ?wheel - wheel ?hub)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (wheel-intact ?wheel)
    |\highlight{\warningcolor}{Syntax error and irrelevant precondition}|
    (not (wheel-deflated ?wheel))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (nut-loosened ?nut))
    (hub-jacked-up ?hub)
    |\highlight{\warningcolor}{Missing precondition: hub unfastened}|
)

Effects:
(and
    (not (wheel-attached ?wheel ?hub))
    (wheel-detached ?wheel)
    |\highlight{\warningcolor}{Missing effect: robot holds the wheel}|
)

==> results/tyreworld_gpt35_pddl/tighten_nut.tex <==
Parameters:
1. ?x - nut: the nut to tighten
2. ?y - hub: the hub in which the nut is located
|\highlight{\warningcolor}{Missing parameter: ?z, the wrench}|

Preconditions:
(and
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (robot-holding ?x))
    (not (hub-jacked-up ?y))
    (nut-in-hub ?x ?y)
    |\highlight{\warningcolor}{Syntax error}|
    (tool-type ?z wrench)
    (robot-holding ?z)
    |\highlight{\warningcolor}{Missing precondition: nut ?x is loosened}|
)

Effects:
(and
    (not (nut-loosened ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (robot-holding ?z))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (lid ?z))
    (nut-in-hub ?x ?y)
)

==> results/tyreworld_gpt35_pddl/unfasten.tex <==
Parameters:
1. ?x - hub: the hub to unfasten
|\highlight{\warningcolor}{Missing parameter: ?y, the nut in the hub}|

Preconditions:
(and
    (hub-jacked-up ?x)
    (nut-in-hub ?y ?x)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (tool-type ?z wrench)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (robot-holding ?z)
    |\highlight{\warningcolor}{Incorrect precondition}|
    (not (nut-loosened ?y))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (wheel-attached ?w ?x)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (wheel-intact ?w)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (wheel-deflated ?w))
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (object-in-container ?z ?c)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (container-open ?c)
    |\highlight{\warningcolor}{Irrelevant precondition}|
    (not (= ?z ?y))
)

Effects:
(and
    (not (nut-in-hub ?y ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (not (wheel-attached ?w ?x))
    |\highlight{\warningcolor}{Incorrect effect}|
    (wheel-detached ?w)
    |\highlight{\warningcolor}{Incorrect effect}|
    (nut-loosened ?y)
    (robot-holding ?y)
    |\highlight{\warningcolor}{Missing effect: hub unfastened}|
)

==> results/tyreworld_gpt4_correction/inflate.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?w - wheel: the wheel to inflate

Preconditions:
(and
    (is-wheel ?w)
    (robot-holding ?w)
    (wheel-deflated ?w)
    (wheel-intact ?w)
    |\highlight{\warningcolor}{Missing precondition: the robot should have a pump}|
)

Effects:
(and
    (not (wheel-deflated ?w))
    (wheel-inflated ?w)
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There is an error in the PDDL model:
1. You allow the robot to inflate a wheel without having a pump, this is incorrect.

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?w - wheel: the wheel to inflate
2. ?p - pump: the pump to inflate the wheel

Preconditions:
(and
    (is-wheel ?w)
    (is-pump ?p)
    (robot-holding ?w)
    (robot-holding ?p)
    (wheel-deflated ?w)
    (wheel-intact ?w)
)

Effects:
(and
    (not (wheel-deflated ?w))
    (wheel-inflated ?w)
)

New Predicates:
No newly defined predicate
----------------------------------------
|\highlight{\inputcolor}{Automated corrective feedback:}|
There is an error in the PDDL model:
1. There is an unknown object type `pump` for the parameter ?p

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?w - wheel: the wheel to inflate
2. ?p - small_object: the pump to inflate the wheel

Preconditions:
(and
    (is-wheel ?w)
    (is-pump ?p)
    (robot-holding ?w)
    (robot-holding ?p)
    (wheel-deflated ?w)
    (wheel-intact ?w)
)

Effects:
(and
    (not (wheel-deflated ?w))
    (wheel-inflated ?w)
)

==> results/tyreworld_gpt4_correction/unfasten.tex <==
|\highlight{\inputcolor}{User:}|
...
The original prompt for PDDL construction
...
Parameters:
-------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
Parameters:
1. ?h - hub: the hub to unfasten
2. ?n - nut: the nut to detach from the hub

Preconditions:
(and
    (is-hub ?h)
    (is-nut ?n)
    (nut-in-hub ?n ?h)
    (nut-loose ?n)
    (hub-jacked-up ?h)
    |\highlight{\warningcolor}{Incorrect precondition: the robot should not hold the nut if the nut is in the hub}|
    (robot-holding ?n)
)

Effects:
(and
    (not (nut-in-hub ?n ?h))
    (hub-unfastened ?h)
    |\highlight{\warningcolor}{Missing effect: the robot should hold the nut at the end}|
)
----------------------------------------
|\highlight{\inputcolor}{Corrective feedback:}|
There are some errors in the PDDL model:
1. There is an incorrect precondition: the robot is not holding the nut because the nut is in the hub
2. There is a missing effect: the robot should hold the nut at the end

Please revise the PDDL model (and the list of predicates if needed) to fix the above errors (and other potentially similar errors).

Parameters:
----------------------------------------
|\highlight{\inputcolor}{GPT-4:}|
1. ?h - hub: the hub to unfasten
2. ?n - nut: the nut to detach from the hub

Preconditions:
(and
    (is-hub ?h)
    (is-nut ?n)
    (nut-in-hub ?n ?h)
    (nut-loose ?n)
    (hub-jacked-up ?h)
)

Effects:
(and
    (not (nut-in-hub ?n ?h))
    (hub-unfastened ?h)
    (robot-holding ?n)
)

==> results/tyreworld_gpt4_pddl/close_container.tex <==
Parameters:
1. ?c - container: the container to close

Preconditions:
(and
    (container-open ?c)
)

Effects:
(and
    (not (container-open ?c))
    (container-closed ?c)
)

==> results/tyreworld_gpt4_pddl/fasten.tex <==
Parameters:
1. ?h - hub: the hub to fasten
2. ?n - nut: the nut to install in the hub

Preconditions:
(and
    (is-hub ?h)
    (is-nut ?n)
    (robot-holding ?n)
    (hub-jacked-up ?h)
    (hub-unfastened ?h)
    |\highlight{\minorcolor}{Unnecessary precondition}|
    (not (nut-in-hub ?n ?h))
)

Effects:
(and
    (not (robot-holding ?n))
    (nut-in-hub ?n ?h)
    (not (hub-unfastened ?h))
    |\highlight{\warningcolor}{Missing effect: the nut should be loose}|
)

==> results/tyreworld_gpt4_pddl/fetch_from_container.tex <==
Parameters:
1. ?x - small_object: the object to fetch from the container
2. ?c - container: the container from which the object is fetched

Preconditions:
(and
    (container-open ?c)
    (object-in-container ?x ?c)
)

Effects:
(and
    (not (object-in-container ?x ?c))
    (robot-holding ?x)
)

==> results/tyreworld_gpt4_pddl/inflate.tex <==
Parameters:
1. ?w - wheel: the wheel to inflate

Preconditions:
(and
    (is-wheel ?w)
    (robot-holding ?w)
    (wheel-deflated ?w)
    (wheel-intact ?w)
    |\highlight{\warningcolor}{Missing precondition: the robot should have a pump}|
)

Effects:
(and
    (not (wheel-deflated ?w))
    (wheel-inflated ?w)
)

==> results/tyreworld_gpt4_pddl/jack_down.tex <==
Parameters:
1. ?h - hub: the hub to jack down
2. ?j - small_object: the jack used to jack down the hub

Preconditions:
(and
    (is-hub ?h)
    (is-jack ?j)
    (robot-holding ?j)
    (hub-jacked-up ?h)
)

Effects:
(and
    (not (hub-jacked-up ?h))
    (hub-on-ground ?h)
)

==> results/tyreworld_gpt4_pddl/jack_up.tex <==
Parameters:
1. ?h - hub: the hub to jack up
2. ?j - small_object: the jack to use for jacking up the hub

Preconditions:
(and
    (is-hub ?h)
    (hub-on-ground ?h)
    (is-jack ?j)
    (robot-holding ?j)
)

Effects:
(and
    (not (hub-on-ground ?h))
    (hub-jacked-up ?h)
)

==> results/tyreworld_gpt4_pddl/loosen_nut.tex <==
Parameters:
1. ?n - nut: the nut to be loosened
2. ?h - hub: the hub where the nut is located
3. ?w - tool: the wrench to be used for loosening the nut

Preconditions:
(and
    (is-nut ?n)
    (is-hub ?h)
    (is-wrench ?w)
    (nut-in-hub ?n ?h)
    (hub-on-ground ?h)
    (robot-holding ?w)
)

Effects:
(and
    (nut-loose ?n)
)

==> results/tyreworld_gpt4_pddl/open_container.tex <==
Parameters:
1. ?c - container: the container to open

Preconditions:
(and
    (container-closed ?c)
)

Effects:
(and
    (not (container-closed ?c))
    (container-open ?c)
)

==> results/tyreworld_gpt4_pddl/predicates.tex <==
1. (container-closed ?c - container): true if the container ?c is closed
2. (container-open ?c - container): true if the container ?c is open
3. (object-in-container ?x - small_object ?c - container): true if the small_object ?x is inside the container ?c
4. (robot-holding ?x - small_object): true if the robot is holding the small_object ?x
5. (is-wrench ?x - small_object): true if the small_object ?x is a wrench
6. (is-nut ?x - small_object): true if the small_object ?x is a nut
7. (is-hub ?x - hub): true if the object ?x is a hub
8. (nut-in-hub ?n - nut ?h - hub): true if the nut ?n is in the hub ?h
9. (hub-on-ground ?h - hub): true if the hub ?h is on the ground (not jacked-up)
10. (nut-loose ?n - nut): true if the nut ?n is loosened
11. (is-jack ?x - small_object): true if the small_object ?x is a jack
12. (hub-jacked-up ?h - hub): true if the hub ?h is jacked up (not on the ground)
13. (hub-unfastened ?h - hub): true if the hub ?h is unfastened
14. (is-wheel ?x - small_object): true if the small_object ?x is a wheel
15. (wheel-on-hub ?w - wheel ?h - hub): true if the wheel ?w is on the hub ?h
16. (is-pump ?x - small_object): true if the small_object ?x is a pump
17. (wheel-intact ?w - wheel): true if the wheel ?w is intact
18. (wheel-deflated ?w - wheel): true if the wheel ?w is deflated
19. (wheel-inflated ?w - wheel): true if the wheel ?w is inflated

==> results/tyreworld_gpt4_pddl/put_container.tex <==
Parameters:
1. ?x - small_object: the object to put into the container
2. ?c - container: the container to put the object into

Preconditions:
(and
    (robot-holding ?x)
    (container-open ?c)
)

Effects:
(and
    (not (robot-holding ?x))
    (object-in-container ?x ?c)
)

==> results/tyreworld_gpt4_pddl/put_wheel.tex <==
Parameters:
1. ?w - wheel: the wheel to put on the hub
2. ?h - hub: the hub to put the wheel on

Preconditions:
(and
    (robot-holding ?w)
    (is-wheel ?w)
    (is-hub ?h)
    (hub-jacked-up ?h)
    (hub-unfastened ?h)
    (not (wheel-on-hub ?w ?h))
)

Effects:
(and
    (not (robot-holding ?w))
    (wheel-on-hub ?w ?h)
)

==> results/tyreworld_gpt4_pddl/remove_wheel.tex <==
Parameters:
1. ?w - wheel: the wheel to remove
2. ?h - hub: the hub from which the wheel is to be removed

Preconditions:
(and
    (is-wheel ?w)
    (is-hub ?h)
    (wheel-on-hub ?w ?h)
    (hub-jacked-up ?h)
    (hub-unfastened ?h)
)

Effects:
(and
    (not (wheel-on-hub ?w ?h))
    (robot-holding ?w)
)

==> results/tyreworld_gpt4_pddl/tighten_nut.tex <==
Parameters:
1. ?n - nut: the nut to tighten
2. ?h - hub: the hub where the nut is to be tightened
3. ?w - tool: the wrench to use for tightening the nut

Preconditions:
(and
    (is-nut ?n)
    (is-hub ?h)
    (is-wrench ?w)
    (robot-holding ?w)
    (nut-in-hub ?n ?h)
    (hub-on-ground ?h)
    (nut-loose ?n)
)

Effects:
(and
    (not (nut-loose ?n))
)

==> results/tyreworld_gpt4_pddl/unfasten.tex <==
Parameters:
1. ?h - hub: the hub to unfasten
2. ?n - nut: the nut to detach from the hub

Preconditions:
(and
    (is-hub ?h)
    (is-nut ?n)
    (nut-in-hub ?n ?h)
    (nut-loose ?n)
    (hub-jacked-up ?h)
    |\highlight{\warningcolor}{Incorrect precondition: the robot should not hold the nut if the nut is in the hub}|
    (robot-holding ?n)
)

Effects:
(and
    (not (nut-in-hub ?n ?h))
    (hub-unfastened ?h)
    |\highlight{\warningcolor}{Missing effect: the robot should hold the nut at the end}|
)
